GRAFS: Graphical Faceted Search System to Support Conceptual Understanding in Exploratory Search

When people search for information about a new topic within large document collections, they implicitly construct a mental model of the unfamiliar information space to represent what they currently know and guide their exploration into the unknown. Building this mental model can be challenging as it requires not only finding relevant documents, but also synthesizing important concepts and the relationships that connect those concepts both within and across documents. This paper describes a novel interactive approach designed to help users construct a mental model of an unfamiliar information space during exploratory search. We propose a new semantic search system to organize and visualize important concepts and their relations for a set of search results. A user study ($n=20$) was conducted to compare the proposed approach against a baseline faceted search system on exploratory literature search tasks. Experimental results show that the proposed approach is more effective in helping users recognize relationships between key concepts, leading to a more sophisticated understanding of the search topic while maintaining similar functionality and usability as a faceted search system.

==> tex/discussion_v1.tex <==
\section{Design Implications}

\subsection{Data model designed for exploratory search}

Our results demonstrate some important implications of designing data representation of a large document set. 

First, our result shows that it is beneficial to capture and show the relation between concepts (or show knowledge subgraph) in the exploration stage. Our results partly support our hypothesis that seeing relations between concepts help people develop deeper understanding of the topic (Section 5.3). Participants subjective feedback also indicates that they appreciate that they are shown the relations explicitly through visualization (Section 5.5, 5.6). This implies that learning the relations between important concepts might serve an important part in people's exploration (may need some citation). 

Second, our study demonstrate that it's important to consider the trade-off between the completeness of the presented information and the usability of the system. Too much information is not appropriate for initial exploration. Treemap provides more complete picture, but is harder to understand. Such components require deeper understanding of the topic.
% Besides, participants' feedback and search outcome implicitly show that seeing the relation between concepts helped participants develop deeper understanding (depth of the outline) and stimulated new ideas (stimulating) (RQ3).
% In our data model, both per-query KG and concept clustering were designed to represent the relations between concepts. In the user study, the two components were most frequently mentioned to be useful by around half of the participants. The quantitative analysis on questionnaire results also proved that participants appreciate the fact that they are shown the relations explicitly through visualization. 

Third ?, we believe the designed data model should be constructed in a per-query manner instead of adapting a pre-defined structure. A per-query data model has two benefits: (1) the selected concepts shown to the users are specific to the search topic, (2) query specific relations might be discovered. For instance, the concept of "Diagnosis" were selected to shown for both "Treatment for depression" and "COVID-19 diagnosis". A pre-defined knowledge graph would give the same set of related concepts starting from "Diagnosis". However, the related concepts given in GRAFS have no overlap between the two topics. The most related concept for "Treatment for depression" is "Depressive Symptoms", while that for "COVID-19 diagnosis" is "Contagious Disease".

% the relation between concepts might be different under different context.
% Per-query KG and concept clustering were designed to represent the relations between concepts. An important question is what role does understanding the relation between concepts play in people's exploration? Our results show that people appreciated the ability of seeing the relations. Besides, participants' feedback and search outcome implicitly show that seeing the relation between concepts helped participants develop deeper understanding (depth of the outline) and stimulated new ideas (stimulating) (RQ3). Based on the result, 

% However, relations didn't have effects on generating an overview of the topic based on our user study.

% Our results suggest that both per-query KG (surfaced using \textit{concept arcs}) and per-query concept clustering (surfaced using \textit{concept treemap}) helped participants see the relation between concepts (RQ2).

Our study also suggests that it's important to preserve human agency in the construction of the data model. In GRAFS, we allow users to make adjustment to the automatically generated data model by deleting or adding concepts. Though this feature was less used in the study, it is one of the most mentioned components when participants talked about the benefits of GRAFS. The use cases provided by participants show that they adjust the concept list based on their exploratory focus, such as things they want to ignore, to keep track of, and to look deeper. We believe this feature will be more widely used in actual exploratory search, as many participants (n=7) mentioned that they didn't edit the concept list because of either time limitation or lack of familiarity with the topic. This feature might be especially useful for users with domain knowledge as they can merge their existing knowledge into the automatically generated data model.


\subsection{User interface design}
We introduced three components in GRAFS, \textit{concept arcs}, \textit{concept treemap}, and \textit{concept grounding}. We observed the benefits of those components and their possible drawbacks. Here we discuss some trade-offs of using those individual components. 
% simplicity and familiarity 
Our results suggest that both \textit{concept arcs} and \textit{concept treemap} are good attempts of surfacing concept relations. One question mentioned by a few users is which component is more effective. Our study shows that \textit{concept arcs} is more intuitive to use and has more direct effects on people's exploration compared to \textit{concept treemap}. \textit{Concept arcs} is used most often in the study, and a majority of participants using \textit{concept arcs} mentioned that it provided hints for the next step of their exploration. This direct effect can encourage users to explore more concepts, but may also become distracting if the relation doesn't make sense to the user or appears repeatedly. \textit{Concept treemap} appears to be difficult to make sense of. Participants' comments regarding usability suggests that \textit{concept treemap} tends to convey too much information. However, among participants that directly compare \textit{concept arcs} to \textit{concept treemap}, five out of seven select \textit{concept treemap}. This suggests that \textit{concept treemap} might be more effective if the user were able to understand information from it. This advantage might come from the overview provided by the \textit{concept treemap}. Users can learn the volume of each concepts, the relative distance between concepts, and the co-occurrence frequency, and therefore develop better understanding of the relation between concepts.

We also found that per-query concept grounding is useful for understanding in the case when the user is not familiar with the concept. Concept grounding was designed to provide an example in the search context by extracting sentences where the concept is used. Participants' qualitative feedback suggests that the provided examples were not helpful and even distracting when the participants already had good background or only focused on familiar concepts during their exploration. Some participants preferred direct explanation from a separate search or a larger context, such as the original articles. As the need for explanation varies between users, a possible solution is to only show concept grounding upon request, and to allow easy connection from concept grounding to a new search query and the original article.

% One of our design goal is to preserve the simplicity, familiarity, and capability of a search interface. Therefore, the visualization components are not dominant in GRAFS. Our result shows that this design largely preserves the normal function of a faceted search interface, while providing better exploration experience and insights for users. Users are free to choose the visualization components to use and ignore during their search. We observed participants that used GRAFS as a Google-like search engine or ignored part of the visualizations such as arcs and treemaps. It is beneficial to give users the freedom to ignore components for tasks that they are somehow familiar with.


\subsection{Limitations and challenges}
\subsubsection{Limitations of the system}
The proposed data model and visualization elements have two limitations: (a) they introduce complexity to users' search when trying to present richer information, (b) they are less familiar to users compared to a typical faceted search interface, so it's hard to get adapted. To cope with those limitations, we built our system on top of a typical faceted search interface and only added visualization to the marginal areas of the interface. We attempted to preserve the simplicity and familiarity of the system, and gave users the freedom to ignore additional components. Our study suggests that GRAFS didn't slow people down when they lookup articles. In terms of subjective perception, participants indicated that GRAFS is less manageable compared to a typical faceted search interface but is similar to the baseline in "easy to use". We observed participants that used GRAFS as a Google-like search engine or ignored part of the visualizations such as arcs and treemaps.

\subsubsection{Limitations of the user study}
Two main limitations of the user study were (a) large impact of the search topic and participants' background, and (b) its time constraint. First, participants' background and topic difference may have much larger influence on the study outcomes than the system, especially for a challenging task involving searching, reading, and writing skills. Therefore, we used a within-subject design and combined objective and subjective evaluation. Second, it takes time for users to make-sense of the visualized information. Under time pressure, they might be discouraged to use those unfamiliar tools and instead use their familiar approach of doing the task. Even when participants were willing to use visualization components, it also required time to fit the new information into their task and writing. We may seek more thorough understanding of the system's usability by observing people using the system to do real-world tasks.

% When faced with a new interface for a relatively familiar task, accepting the new tool is challenging. Therefore, it is beneficial to give users the freedom to ignore components or 
% While providing richer information, the proposed data model and visualization elements may also introduce complexity in users' understanding and exploration. One of our design goal is to preserve the simplicity, familiarity, and capability of a search interface. Therefore, the visualization components are not dominant in GRAFS. Our study suggests that the additional information didn't slow people down when they lookup articles. In terms of subjective perception, participants indicated that GRAFS is less manageable compared to a typical faceted search interface. 

% \begin{itemize}
%     \item data model
%     \begin{itemize}
%         \item enough for an overview?
%         \item the role of ontology in our project
%         \item generalize to other domain, other profession
%         \item reading more articles in the baseline system?
%     \end{itemize}
%     \item interface design
%     \begin{itemize}
%         \item visual hint of interesting elements
%         \item compare to baseline
%     \end{itemize}
%     \item user study
%     \begin{itemize}
%         \item lots of factors influence the outcome, background knowledge
%         \item the usefulness of components can only be seen when used for longer time 
%         \item adaptation to features, learning effects
%     \end{itemize}
%     \item user behavior? need some search log analysis
% \end{itemize}

==> tex/experiment_v1.tex <==
\section{Experimental Evaluation}
We conducted a controlled user study to evaluate the usability of GRAFS and its ability to facilitate exploratory search and learning. We compared GRAFS to a typical faceted search UI with the same set of facets and documents to understand the effects of the newly introduced knowledge subgraph and visualization components. 
% Results from the experimental tasks and feedback from post-study questionnaires and interviews suggest that GRAFS helped users see the relation between concepts and improved exploratory search. Results also illustrate the challenges presented for evaluating systems designed for exploratory tasks.

\subsection{Hypotheses}
\label{sec:Hypotheses}
The user study was designed to test the following hypotheses:

\textbf{Hypothesis 1.} With the help of the knowledge subgraph, GRAFS positively influences users' conceptual understanding and sensemaking activities.
\label{hyp1}
\begin{itemize}
    \item [\textbf{1.a}] We expect GRAFS to help users develop a better understanding of concept relations compared to the baseline system. The graphicl \textit{facet list} and \textit{facet treemap} present relations between concepts in the current searching context and an overview of the large information space, which may otherwise require a substantial effort to build mentally via manual search and inference. %Q1, Q2
    \item [\textbf{1.b}] Seeing concept relations helps users gain deeper understanding of the search topic during sensemaking. Knowing concept relations should help users build better a conceptual understanding and mental model of the topic, and encourage users to explore more deeply into the results.
    % sensemaking/learning (understanding?): A1, A3, A5
    % search/gathering/foraging (exploration?): Q3, Q4, A2, A5
    % overall: A6, I1, I4
\end{itemize}

\textbf{Hypothesis 2.} The additional complexity introduced in GRAFS has no negative influence on users' searching activity. %Q5, time cost
\label{hyp2}
\begin{itemize}
    \item [\textbf{2.a}] We expect that the introduction of the additional features in GRAFS will not hurt people's performance in facet filtering tasks. GRAFS preserved the layout and functionality of a faceted search interface, so users should be able to perform filtering tasks as in a typical faceted search interface. %Q5, time cost
    \item [\textbf{2.b}] We expect the complexity of additional information provided in GRAFS will not hurt the overall usability of the system. The proposed data model and interface design present the concept relation information in a simplified way that facilitates users' learning and understanding of those complex information.
    % Q6 - Q9
    % I3, I4
    % I5
    % GRAFS preserved the simplicity of a typical faceted search interface, leveraging the usability of a familiar system.
\end{itemize}

% \textbf{Hypothesis 3.} We expect the (complexity) additional features in GRAFS won't hurt the overall usability of the system and people's performance in faceted filtering task. GRAFS preserved the layout and functionality of a faceted search interface, leveraging the usability of a familiar system.



% \textbf{Research questions:} Compared to a traditional faceted search interface
% objective task1: outline overview. 
% find concepts
% relations, conceptual understanding.
% task2: finding by faceting. does the new interface help users as effectively as the old one?
% questionnaires/interview: subjective feelings

% \begin{itemize}
% % \item will the contextual tool-tip feature help a user better understand and use the facets
%     \item Will GRAFS help users learn an overview of the search topic?
%     \item Will GRAFS help users better develop conceptual understanding of the search topic, including the major concepts and how they are connected?
%     \item Will GRAFS encourage users to explore the search results deeper?
%     \item Will customizable facets better fit the user's need as a tool not just for filtering, but also learning?
%     \item In what situation/tasks will a traditional faceted search interface be more effective than GRAFS?
%     \item What visualization components are effective for exploratory search?
% \end{itemize}
\subsection{Study Design}

\subsubsection{Overview}

We adopt a within-subject design ($N=20$) where each participant is exposed to two Web-based search interface conditions, GRAFS and the baseline, working on two topics (``COVID-19 Diagnosis'' and ``Treatment for Depression''). Users were randomly split into two groups of 10 to either work on (a) COVID-19 + GRAFS and Depression + Baseline, or (b) COVID-19 + Baseline and Depression + GRAFS. To alleviate the learning effect, we also counter-balanced the order of interface conditions and search topics. In other words, half of the users in condition (a) worked on GRAFS first and the baseline next, and same for users in condition (b).

\subsubsection{Search Tasks}
Participants were asked to imagine being tasked to write a survey paper on either COVID-19 Diagnosis or Treatment for Depression. Given a search system and query, such as GRAFS and COVID-19 Diagnosis, participants needed to complete two tasks: (1) produce an outline for the hypothetical paper (30 minutes), and (2) answer questions about specific aspects of the topic by facet filtering (10 minutes). 


\textbf{Task 1: Outline Generation}. For the outline task, participants were asked to use the gathered information to generate an outline of the hypothetical paper. Given the time limitation, we suggested to participants that they should produce outlines in the form of bullet points with indentations that indicate the structure rather than organized, well-written paragraphs. Participants were instructed to provide sub-topics, major arguments or short descriptions for each sub-topic, and document references in their outlines to reflect the overall structure of the hypothetical paper. 

\textbf{Task 2: Question Answering.} The outline task evaluates users' exploration on a broad topic, which is often not how faceted search is primarily used. We therefore included a question-driven task where participants focus on looking up answers for the following specific questions. 

\begin{itemize}
    \item \textit{COVID-19 Diagnosis:} Find evidence that antibody can be used to detect asymptomatic COVID-19 infection.
    \item \textit{Treatment for Depression:} Find if there are any clinical trials that study the effects of antidepressant medication.
\end{itemize}

Participants were given 10 minutes to find one or two articles that can answer the given question. They were not required to summarize the found articles.

\textbf{Rationale for Selecting the Search Topics:} As most of our participants are not from the biomedical domain, well-known health-related topics with relatively easy terminologies are favorable. Both COVID-19 and Depression are familiar topics for laypeople, and they also involve professional concepts in the biomedical literature that require learning and exploration. Therefore, we chose these two topics so that participants could start their exploration quickly and have the potential to learn unfamiliar concepts. 

\subsubsection{Participants}
We recruited 20 participants ($male=10$, $female=10$) via campus-wide mailing lists. All participants either were pursuing or had attained a graduate degree in a STEM field. Six participants had a biomedical background or professional experience, such as working as a Molecular Biology researcher. Participants were randomly assigned to different conditions.

\subsubsection{Procedure}
User study sessions were conducted either in-person or remotely using Zoom video conferencing, and each lasted for roughly two hours. After providing informed consent, participants completed a demographics questionnaire that asked about their background and prior experience with literature search. A study session contained two sub-sessions that followed the same sequence of steps and a participant completed the outline task and question answering task on one topic using one interface design in each sub-session. At the beginning of a sub-session, we guided the participant through a hands-on tutorial of the search interface using an example topic. Participants were then informed of the topic to work on and asked to rate their level of familiarity with the topic on a scale from 1 (unfamiliar) to 7 (familiar). Then, participants completed the outline and question answering task. After the two tasks, participants finished a post-task questionnaire to provide feedback for the search interface. Finally, after completing the two sub-sessions, participants provided additional feedback about their experience using the tools through an exit interview.

\subsubsection{Outcome Measures}

We evaluated the system using both subjective feedback from users and an objective evaluation of the generated outlines.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{User Perceptions:} In the post-task questionnaire after each sub-session, participants provided their level of agreement with nine statements listed in Table \ref{table:post-task}, on a scale from 1 (strongly disagree) to 7 (strongly agree). These questions are shown in Table \ref{table:post-task}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Outline Generation Task:} To test \textbf{Hypothesis 1}, we evaluated the quality of participant generated outlines according to six rubric items as listed in Table \ref{table:outline}. A1, A2, and A3 focus on the system's effect on sensemaking and learning, while A4 and A5 focus on the effect on people's searching and foraging. Three graders were asked to select the better outline between the two generated by each user on all of the criteria. The graders were not informed of the system used to generate the outlines and did the grading independently. In the end, we counted the total number of votes given to each system on each criterion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Question Answering Task:} For the question answering task, we focused on measuring the time spent for participants to find satisfactory articles.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\textbf{Qualitative User Feedback:} We asked for detailed feedback using a semi-structured exit interview with the questions in Table \ref{tab:interview}.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\begin{tabular}{llll}
\toprule
 & & H & Question \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Outline\\ generation\end{tabular}} & \textbf{Q1 Overview} & 1.b& \begin{tabular}[c]{@{}l@{}}The faceted search tool helped me gain an overview \\ of key concepts in the search results.\end{tabular} \\ \cmidrule{2-4} 
 & \textbf{Q2 Relation} & 1.a& \begin{tabular}[c]{@{}l@{}}The faceted search tool helped me see how \\ key concepts are related in the search results.\end{tabular} \\ \cmidrule{2-4} 
 & \textbf{Q3 Discover} & 1.b & \begin{tabular}[c]{@{}l@{}}The faceted search tool helped me discover interesting \\ aspects to explore further.\end{tabular} \\ \cmidrule{2-4} 
 & \textbf{Q4 Decision} & 1.b & \begin{tabular}[c]{@{}l@{}}The faceted search tool helped me decide which aspects \\ to focus on and which to ignore.\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Question \\ answering\end{tabular} & \textbf{Q5 QA difficulty} & 2.a & \begin{tabular}[c]{@{}l@{}}I find it difficult to use the faceted search tool when I \\ complete the question answering task.\end{tabular} \\ \midrule
\multirow{4}{*}{Usability} & \textbf{Q6 Easy to use} & 2.b& The faceted search tool is easy to use. \\ \cline{2-4} 
 & \textbf{Q7 Manageable} & 2.b & The faceted search tool is manageable. \\ \cmidrule{2-4} 
 & \textbf{Q8 Stimulating} & 2.b & The faceted search tool is stimulating. \\ \cmidrule{2-4} 
 & \textbf{Q9 Well-organized} & 2.b & The faceted search tool is well-organized. \\ \bottomrule
\end{tabular}
\caption{Post-task questionnaire.}
\label{table:post-task}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\begin{tabular}{llll}
\toprule
 & & H & Description \\ \midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}l@{}}Sensemaking/\\ Learning\end{tabular}} & \textbf{A1 Structure} & 1.a, 1.b & \begin{tabular}[c]{@{}l@{}}Which outline is more logically organized\\/structured, as opposed to a list of randomly\\ ordered points?\end{tabular} \\ \cmidrule{2-4} 
 & \textbf{A2 Interpretation} & 1.b & \begin{tabular}[c]{@{}l@{}}Which outline contains more interpretation \\written by users?\end{tabular} \\ \cmidrule{2-4} 
 & \textbf{A3 Topical depth} & 1.b & \begin{tabular}[c]{@{}l@{}}Which outline covers deeper issues of the \\ topic, as opposed to superficial issues?\end{tabular} \\ \midrule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Search/\\ Foraging\end{tabular}} & \textbf{A4 Documentation} & 1.b & \begin{tabular}[c]{@{}l@{}}Which outline collects more papers to \\ document their findings?\end{tabular} \\ \cmidrule{2-4} 
 & \textbf{A5 Topical diversity} & 1.b & \begin{tabular}[c]{@{}l@{}}Which outline covers more diverse issues, as \\ opposed to being narrowly focused?\end{tabular} \\ \midrule
 & \textbf{A6 Overall} &1.a, 1.b& \begin{tabular}[c]{@{}l@{}}Which outline is overall the better one of the\\ two?\end{tabular} \\ \bottomrule
\end{tabular}
\caption{Outline assessment rubric.}
\label{table:outline}
\end{table}



% the list of interview questions
\begin{table}[h]
\begin{tabular}{lll}
\toprule
&H& Description\\\midrule

\textbf{I1 Subjective outline evaluation} & 1 & Which outline are you more satisfied with?                                                                                                                \\\midrule
\textbf{I2 General strategy}              & 1 & Could you describe your strategy for approaching the task?                                                                                                    \\\midrule
\textbf{I3 Benefit of each system}        & 1, 2 & \begin{tabular}[c]{@{}l@{}}Did either of the faceted search tools help you in any way \\ to accomplish the task? If so, how? If not, why not?\end{tabular} \\\midrule
\textbf{I4 GRAFS vs baseline}             &1, 2& \begin{tabular}[c]{@{}l@{}}If you were to do the same task again, which of the two\\ interfaces would you prefer to use? Why?\end{tabular}                   \\\midrule
\textbf{I5 Per-component usability}       & 2.b& \begin{tabular}[c]{@{}l@{}}Did you find \{concept arcs, treemap, example tooltip, \\ deleting, adding\} useful? Why?
\end{tabular}  \\\bottomrule
\end{tabular}
\caption{Exit interview questions.}
\label{tab:interview}
\end{table}


% regarding (1) usability of different features of GRAFS, (2) the benefits of each system and participants' preference between the two, (3) quality of the generated outline. (need reference?) 











==> tex/method_v1.tex <==
\section{Graphical Faceted Search}
\label{sec:Graphical Faceted Search}
In this section, we describe the design and implementation of the graphical faceted search (GRAFS) system. We start by motivating our research problem. We then divide the problem into two parts: a data representation problem and an interactive presentation problem. In each part, we formulate the problem, discuss the general solution framework, and describe our specific implementation of the solution.

\subsection{Challenge and Motivation}

An exploratory searcher needs to obtain an overview of a large number of potentially relevant documents returned by her query. Instead of reading these documents one by one trying to build the conceptual understanding of the information space, a better strategy is to learn key concepts and relations that show up frequently throughout the search results. In fact, semantic search engines also generate and leverage such information in their backend~\cite{reinanda2020knowledge}.

\begin{figure}
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.76\linewidth]{fig/Thalia.pdf}
  \caption{Faceted filters}
  \label{fig:challenge-facet}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=.85\linewidth]{fig/entity-graph.pdf}
  \caption{Knowledge subgraph visualization}
  \label{fig:challenge-vis}
\end{subfigure}
\caption{Challenges in presenting concepts and relations in search results. (a) A screenshot of Thalia search engine's result page for the query ``treatment for depression'' over PubMed abstracts~\cite{soto2019thalia}. Hundreds of MeSH terms and UMLS concepts mentioned in the search results are used as faceted filters. This leads to exceedingly long lists of faceted filters on two sides of the interface. (b) A visualization of the knowledge subgraph constructed for the query ``Zika fever'' on English Wikipedia (reproduced with author's permission) ~\cite{dietz2019ent}. Each node is a DBpedia concept mentioned in the search results. Two concepts are connected by an edge if they are mentioned in the same context in any search result. Showing all relationship links is visually overwhelming even after pruning the number of concepts down to two dozen. }
\label{fig:challenge}
\end{figure}

A semantic search engine applies entity recognition and linking algorithms to documents (at index time) and queries (at search time). This has become increasingly common thanks to the advances in natural language processing (NLP) and the availability of knowledge graphs  (also called standardized vocabularies or ontologies) in different domains. As a result, when a search engine returns a list of documents, it can simultaneously return a set of entities (and their relations) recognized in these documents. In other words, a semantic search not only returns a set of documents, but also a set of semantic units, a subgraph inside the global knowledge graph. On the one hand, this knowledge subgraph has great potential to help an exploratory searcher obtain a mental model of the information space in question. On the other hand, this knowledge subgraph can be enormous if it is shown in its raw form. It may consist of not only core concepts of the information space, but also a large number of peripheral and even non-relevant concepts that happen to be mentioned in the result documents. Therefore, \textbf{it is challenging to allow exploratory searchers make use of a query-specific knowledge subgraph in a non-overwhelming manner.} 

To illustrate this challenge, consider NaCTeM's Thalia search system for PubMed abstracts~\cite{soto2019thalia}. The system uses NLP algorithms to extract UMLS concepts and MeSH terms from abstracts and use them as faceted filters on the result page. As shown in Figure \ref{fig:challenge-facet}, the query ``treatment for depression'' retrieves an exceedingly long list of concepts from search results, which resulted in faceted filters vertically spanning multiple screens! Even worse, top-ranked concepts in each semantic category (facet) are most frequent yet non-informative, such as  \emph{Human} in \emph{Gene/Species}, \emph{Cell} in \emph{Anatomical Parts}, and \emph{Oxygen} in the category \emph{Chemical}.


To reduce the complexity of the query-specific knowledge subgraph, researchers have proposed selection and ranking algorithms aiming to preserve only a set of core concepts~\cite{dalton2013constructing, schuhmacher2015ranking, dietz2019ent}. However, even after reducing the space of concepts, the number of possible relationships among concepts can still be large. Figure \ref{fig:challenge-vis} shows a knowledge subgraph produced by a state-of-the-art approach when searching Wikipedia articles using the query ``Zika fever''~\cite{dietz2019ent}. Despite having only 24 concepts, the subgraph is densely connected due to intricate relationships between these concepts in search results. Showing all relationship links upfront can easily overwhelm a user's mind.

The above challenge directly motivates our work. Below we describe our approach to this challenge, including computational methods for constructing and maintaining a knowledge subgraph for exploratory search, as well as interactive designs for presenting the data model to users. As a specific use case, we construct and present knowledge subgraphs to medical literature searchers in an uncluttered and non-overwhelming manner. 

% However, faceted search and concept visualization can easily overwhelm users when the number of concepts and relations present in search results is large. This is increasingly common as natural language processing (NLP) algorithms are applied to identify concepts and relations inside search results from a large ontology. Even though such an interface may be useful for highly skilled domain experts, a user who is learning about the topic for the first time would get swamped and lost in the long, uninformative list of concepts.

% Therefore, when search engines return a list of documents, it also implicitly returns a set of entities and relations mentioned in these result documents. If we take a knowledge graph perspective, these returned entities and relations constitute a subgraph inside a larger encyclopedic knowledge graph. Although this subgraph is specific to a search query, it may contain a large number of entities and relations. Many of which are not central to the understanding of the search topic. For example, (Show examples of Thalia and ENT-Rank).





\subsection{Initial Knowledge Subgraph For Exploratory Search}

In this section, we formulate the problem of constructing an initial knowledge subgraph for exploratory search. We then describe an efficient solution, which supplies the data model used in the interactive interface.

\subsubsection{Problem Formulation}
A semantic search engine returns not only a ranked list of results for a given query, but also concepts (or entities) and their relations within those results. Formally, a search query $q$ retrieves a list of documents $D_q = \{d_i\}_{i=1}^n$. Within each document $d_i$, the search system also recognizes a set of concepts $C_i \in C$ and a set of relations $R_i \in R$. Here, $C$ is the set of all possible concepts in the global knowledge graph, and $R$ is the set of all possible relations between those concepts. Therefore, in addition to the list of documents $D_q$, the search query $q$ effectively retrieves a query-specific knowledge graph $G_q = (C_q, R_q)$, where $C_q = \cup_{i=1}^n C_i$ and $R_q = \cup_{i=1}^n R_i$. We assume that concepts and relations in $G_q$ have been pre-extracted by NLP algorithms in the search engine backend~\cite{dalton2013constructing, wolfe2017pocket, reinanda2020knowledge}. As described in the previous subsection, $G_q$ often contains a large number (hundreds or even thousands) of concepts and relations. Directly presenting the entire graph $G_q$ to users will inevitably cause information overload. 

The problem of constructing an \textbf{initial knowledge subgraph for exploratory search} is to find a small subgraph $H_q \subset G_q$ that is most helpful at the initial stage of an exploratory search task. Just as a traditional search interface tackles information overload by showing a small number (e.g., 10) of the most relevant documents on the first page, we posit that an  exploratory search interface will encourage learning and navigation by showing a small initial subgraph of the most important concepts and relations. As the exploration unfolds, the user will gradually move beyond this initial subgraph.

How to construct such a knowledge subgraph? If our goal is to find a subgraph with $k$ concepts to be shown to the user (where $k$ is small), then it translates into a computational problem of selecting the best $k$-sized subgraph $H_q$ out of the original graph $G_q$. In this work, we adopt the following criteria to guide the selection:
\begin{itemize}
    \item \textbf{Relevance}: Concepts and relations in this subgraph should be centered around the user's search interest, as opposed to drifting into peripheral parts of the information space. 
    \item \textbf{Coverage}: Concepts and relations in this subgraph should cover diverse subregions of the information space, as exploratory search aims at breadth and learning. 
    \item \textbf{Efficiency}: The subgraph selection procedure should be efficient enough to be executed at interactive response rate to support a smooth exploration experience.
\end{itemize}

We note that these criteria are inspired by research on search result diversification~\cite{rodrygo2015search}, where the goal is to provide result documents to cover different aspects of an ambiguous query. In the learning stage of an exploratory search, the user's goal is also ambiguous. The crucial difference is that here our goal is to select or rank knowledge graph concepts instead of result documents.

Even after being pruned to a manageable size, a knowledge graph can still be too abstract to make immediate sense in a user's eyes.  To further support user interpretation of the extracted knowledge subgraph $H_q$, we augment it with the following data elements to be used in the frontend interface.

\begin{itemize}

\item \textbf{Concept Provenance}. For each concept $c \in H_q$, we identify a small representative set of context windows (e.g. sentences) in result documents $D_q$ which mention the concept $c$ and the query $q$. These context windows explain why a concept is relevant in the search context.



\item \textbf{Graph Partitioning}. We partition the set of concepts in $H_q$, such that concepts in the same partition are densely connected by edges in $H_q$, and concepts between partitions are loosely connected by edges in $H_q$. Such partitioning will be useful when visualizing concepts in the frontend. We present semantically related concepts visually close to each other in the interface. This nudges users to think about connections between nearby concepts, according to the proximity principle in Gestalt Principles~\cite{todorovic2008gestalt}.

\end{itemize}

% Constructing and pruning query-specific knowledge graph has attracted much research and applications from the information retrieval community~\cite{google-kg-blog, dalton2013constructing, dietz2019ent}. The resulting knowledge subgraph (also called ``pocket knowledge graph''~\cite{wolfe2017pocket}, ``knowledge sketch'', or ``query-specific knowledge graph''~\cite{dalton2013constructing}) is then used to better interpret user's queries, improve ranking of documents, and support conversational search~\cite{vakulenko2017conversational}. Here our goal is to show this knowledge subgraph in the search interface. This goal places a few constraints. 

% First, the entities and relations are relevant to the search context. Entities and relations should appear in (a large number of) search results. The popularity across search results acts as a natural explanation to users as to why these relations can be relevant.

% Second, the subgraph should cover a wide range of the information space. 

% Third, it has to be efficiently computed to support interactive applications.  



% \begin{wrapfigure}{r}{0.25\textwidth}
%   \begin{center}
%     \includegraphics[width=0.25\textwidth]{fig/Thalia.png}
%   \end{center}
%   \caption{Thalia search engine for PubMed abstracts. MeSH terms and UMLS concepts in all search results are shown as faceted filters. This results in long list of faceted filters.}
% \label{fig:thalia}
% \end{wrapfigure}



% However, faceted search and concept visualization can easily overwhelm users when the number of concepts and relations present in search results is large. This is increasingly common as natural language processing (NLP) algorithms are applied to identify concepts and relations inside search results from a large ontology. As one example, consider the Thalia search engine. The system uses NLP algorithms to extract concepts in UMLS Metathesaurus (a large medical ontology) from search results and use them as faceted filters. As shown in Figure \ref{fig:thalia}, the search query ``treatment for depression'' results in an exceedingly long list of concepts in faceted filter. Even Thalia groups the concepts into multiple facets, there can still be hundreds of concepts under each category. A user needs to scroll multiple screens to see all of them. Top-ranked concepts in each category are frequent yet non-informative, e.g., ``Oxygen'' in the ``Chemical'' category, ``Human'' in ``Gene/Species'', ``Cell'' in ``Anatomical Parts'', and so on. Even though such an interface may be useful for highly skilled domain experts, a user who is learning about the topic for the first time would get swamped and lost in the long, uninformative list of concepts.

% Sensemaking process consists of a learning loop, where the user gradually refines their understanding (mental schema) of the information in a search process. To help users in the sensemaking process, an ideal interface would start by selecting a few most important concepts needed for setting up an initial understanding, and gradually nudge the user to build up an increasingly nuanced understanding of the information space in a progressive manner. Either showing too little or too much information is suboptimal.

% \ray{
% Motivation: ad-hoc semantic search results implicitly contain a (large) knowledge graph. Example: the Thalia search system for PubMed.

% In general, this highlights a problem: in the ad-hoc search process, we implicitly retrieve an associated (raw) knowledge graph. Just as document ranking helps prioritize a large set of retrieved documents, an associated task is to prioritize a large set of knowledge graph elements.

% A diagram:  document set, a large knowledge graph -> presentation: document ranking, knowledge graph ranking -> each node in the subgraph is grounded, subgraph has meaningful partitions

% goal of ad-hoc knowledge subgraph construction
% (1) be relevant to the search context, 
% (2) cover the information space to stimulate learning, and 
% (3) be concise and expandable on-demand so that it does not overwhelm the user upfront. 


% derived tasks of ad-hoc knowledge subgraph construction
% (1) concept grounding: how does a concept in AKS relate to the search query?
% (2) concept clustering: partitioning an AKS into parts to give overview.

% }

% \subsubsection{Problem formulation} 
% We start by defining the following concepts and notations.

% \textbf{Search query}: a search query $q$ is a representation of user's information need, usually expressed as a sequence of terms (from free-text or a controlled vocabulary). 

% \textbf{Semantic document}: a semantic search result consists of $(d, C)$, where $d$ is a document (e.g. unstructured text or semi-structured record), $C$ is a set of concepts appearing in $d$. These concepts are linked to entries in a large controlled vocabulary $V$. That is, $C \subset V$. Each concept $c \in C$ may be grounded in parts of document $d$ either manually by domain experts or automatically by an algorithm. 

% \textbf{Search results}: search results are a ranked list of semantic documents $\{(d_i, C_i)| 1 \le i \le n_q\}$ retrieved by a query $q$. $(d_1, C_1)$ is the first result, $(d_2, C_2)$ is the second result, etc.

% \textbf{Per-query knowledge graph construction}: given query $q$ and the corresponding search results $\{(d_i, C_i)| 1 \le i \le n_q\}$, a knowledge graph of size $k$ consists of a graph $(V_q, E_q)$. $V_q$  is a set of concepts, $V_q \subset \cup_{i=1}^{n_q} C_i$ and $|V_q| = k$. $E_q$ is a set of edges $\{(u,v)| u \in V_q, v \in V_q\}$. These edges represent relations between concepts in the search result of $q$. Optionally, each edge may have a relation type specified by $r: E_q \rightarrow R$ ($R$ is the set of all relation types).

% \textbf{Per-query concept grounding}: given query $q$, the corresponding search results $\{(d_i, C_i)| 1 \le i \le n_q\}$, and the set of concepts $V_q$ in the per-query knowledge graph. The problem of contextual sentence extraction is to identify, for each concept $c \in V_q$, a small representative set of sentences $\{s_c\}$ in search result documents $\{d_i\}$ which mention the concept $c$. 

% \textbf{Per-query concept clustering}: given per-query knowledge graph $(V_q, E_q)$. The problem of per-query concept clustering is to assign cluster identities to concepts $c \in V_q$, such that concepts in the same cluster are densely connected by edges in $E_q$, and concepts between clusters are loosely connected by edges in $E_q$.

% In principle, we aim to represent and summarize the semantic space specific to a search query using a knowledge graph, and facilitate concept and graph understanding using concept grounding and clustering. 

% Compared to a flat concept list, knowledge graphs are often used to store relations between entities, thus containing richer information and a complete picture. We image the process of exploratory search to be a random walk on the knowledge graph, where users traverse through concepts directed by relations that connect concepts. There are existing knowledge graphs constructed by experts or manual labeling. But those knowledge graphs may not fit into the search context and can not show how concepts are related within user's scope of interest. The per-query knowledge graph is based on automatically mined relations and incorporates information specific to the retrieved set of documents. The types of the relations may vary based on the task.

% A smooth exploration experience requires users to have a basic understanding of each entity/concept in the graph. More importantly, users need to see how a concept is related to the topic of interest. The per-query concept grounding is essentially generating an extractive summary of content related to both the concept and the search query. 

% The knowledge graph generated from a document set can be massive and densely connected, making it complicated to explore and hard to start with. It is useful to group strongly related concepts into clusters so that users can focus on one group at a time. Concept clustering helps to generate clusters based on their relations. 

% \begin{itemize}
%     \item why we use semantic document
%     \item Knowledge graphs are often used to store relations between entities (more information than a flat list of concepts)
%     \item Make exploratory search as a directed walk on the knowledge graph based on concept relations.
%     \item Knowledge graph also facilitates the selection of a small subset from the entire set of concepts.
%     \item There are existing knowledge graphs constructed by experts or manual labeling. But those knowledge graphs may not fit into the search context and can not show how concepts are related within user's scope of interest.
%     \item The per-query knowledge graph is based on automatically mined relations and incorporate information specific to the retrieved set of documents. The types of the relations may vary based on the task.
%     \item The per-query concept grounding process aims to provide a quick explanation of a given concept, which helps with understanding of individual concept (node in the knowledge graph).
%     \item Concept clustering add sections to the knowledge graph, serving as a set of automatically generated categories.
%     \item Overall, the core of our data model is the per-query knowledge graph. It can be seen as a succinct summary of the major concepts and their relations specific to a given queryWe further added concept grounding and concept clustering to facilitate concept and graph understanding.
% \end{itemize}

\subsubsection{Implementation}

In principle, one can apply existing methods for ranking and selecting knowledge graph concepts for search tasks~\cite{dalton2013constructing,schuhmacher2015ranking,dietz2019ent}. However, these methods are mainly optimized for batch evaluation settings and their computational cost can be too high to be run at an interactive rate. For example, shortest-path algorithms and random walks on the query-specific knowledge graph $G_q$ has superlinear (e.g., quadratic) time complexity in the number of concepts in $G_q$. We design an efficient implementation as follows.




\textbf{Initial Knowledge Subgraph Construction.} We implemented the described data model on top of a custom-built search engine for 32.6 million PubMed abstracts, which were downloaded from the National Library of Medicine website. We use an efficient maximal pattern matching-based   algorithm~\cite{dai2008efficient,jonquet2009open} to annotate clinical concepts mentioned within each abstract by looking up terms in the SNOMED-CT vocabulary. Given a search query $q$, we first extract the original query-specific knowledge graph $G_q = (C_q, R_q)$ as follows. All concepts mentioned in the set of retrieved documents $D_q$ forms the extracted concept set $C_q$. We take a generic view of concept relations and  assume that a pair of concepts in $C_q$ are  related if they co-occur in any retrieved document. This generates a set of concept relations $R_q$. 

% we leveraged the co-occurrence frequency of concepts in documents with the assumption that concepts mentioned together often are strongly related. Specifically, given two concepts $c_i$ and $c_j$ and two sets of documents $D_i$ and $D_j$ where the two concepts are mentioned respectively, $r_{ij}$ is calculated as $|D_i \cap D_j|$.

We then constructed a subgraph $H_q \in G_q$ that contains a user-specified number (e.g., 20) of concepts in $C_q$. We incorporate the \emph{relevance} and \emph{coverage} criteria into an efficient subset selection algorithm inspired by the maximal marginal relevance ~\cite{carbonell1998use}. The basic idea is to sequentially select items that simultaneously have high relevance to the query and few relationship links between each other.

% Our concept selection criterion was inspired by  ($MMR$). A concept will be assigned with a high score if it is both relevant to the query and has minimum similarity with already-selected concepts (\textbf{Relevance}, \textbf{Coverage}). 

Formally, let $q$ be the search query, $C_i \subset C_q$ be the current set of selected concepts with size $i$ (initially $i=0$, $C_i = \varnothing$), and $C_q\setminus C_i$ be the current set of unseleted concepts. We select the next concept  $c_{i+1}$ as follows:
\begin{equation}
c_{i+1} \leftarrow \argmax_{c \in C_q \setminus C_i} \left[\lambda \cdot r(c, q) - (1-\lambda) \cdot \max_{c_j \in C_i} s(c, c_j) \right] \ . \label{equ:mmr-concept}
\end{equation}
Here, $c$ is a candidate concept in the current set of unseleted concepts. $r(c,q) = |\{d|c \in d, d \in D_q\}|$ measures the \textbf{relevance} of $c$ by the number of retrieved documents containing $c$. $s(c, c_j) = |\{d|c \in d, c_j \in d, d \in D_q\}|$ measures the relationship strength  between $c$ and a selected concept $c_j \in C_i$ by the number of documents where $c$ and $c_j$ co-occur. Intuitively, the term ``$-\max_{c_j \in C_i} s(c, c_j)$'' promotes \textbf{coverage} of the next concept $c$ by forcing it to be semantically far from the current selected set $C_i$. $0 < \lambda < 1$ is a tuning parameter that defines the relative importance of relevance and coverage criteria.
$k$ concepts are added into $H_q$ incrementally following Equation \eqref{equ:mmr-concept}.
The algorithm runs \textbf{efficiently} with time complexity $O(k^2|C_q|)$, a linear (instead of quadratic) complexity in the number of concepts in $G_q$. 


In our implementation, we set $\lambda = 0.5$ to put equal importance on relevance and coverage criteria. We noticed that some selected concepts are frequent but not informative. For instance, the concept ``COVID-19'' appears in more than half of the documents retrieved by a COVID-19 related query, and therefore has a large relevance term $r(c,q)$. However, such a concept contains little new information about the topic. We therefore omitted concepts with $r(c,q) > |D_q|/2$, treating them as equivalent to ``stop words''  (frequent functional words)  in the context of the current search results $D_q$.

\textbf{Concept Provenance.} For each selected concept $c$ in $H_q$, we extracted three representative sentences containing both concept $c$ and query $q$ to show how $c$ is used in the context of search results. The selection algorithm is also inspired by maximal marginal relevance. First, all sentences containing $c$ were extracted from $D_q$ to form the candidate sentence set $S_q$. Let $S_i \in S_q$ be the current set of selected sentences with size $i$ (initially $i=0, S_q = \varnothing$). The algorithm selects the next sentence $s_{i+1}$ as follows:

\begin{equation}
s_{i+1} \leftarrow  \argmax_{s \in S_q \setminus S_i} \left[\lambda \cdot v(s, q) - (1-\lambda) \cdot \max_{s_j \in S_i} v(s, s_j) \right] \ .
\label{mmr-sentence}
\end{equation}
Here, $v(s,q)$  measures the relevance of sentence $s$ with respect to query $q$, while $v(s, s_j)$  measures the similarity between the candidate sentence $s$ and a selected sentence $s_k$. The function $v(\cdot, \cdot)$ represents queries and sentences as bag-of-words vectors with TFIDF weights and computes cosine similarity between two vectors. We empirically set $\lambda = 0.5$ to balance relevance and diversity of the set of selected sentences.

\textbf{Graph Partitioning.} This step generates groups of concepts in $H_q$ based on their relations. Instead of choosing a fixed number of partitions (as in algorithms like $k$-means or $k$-medoids), we performed agglomerative hierarchical clustering over the concepts in $H_q$. First, each concept starts in its own cluster. At each subsequent step, two closest clusters are merged. The distance between two clusters is the distance between the farthest concepts (complete-linkage clustering). The distance between two concepts is calculated as the symmetric difference between the two sets of documents that contain each concept: $d(c_i, c_j) = |D_i \cup D_j| - |D_i \cap D_j|$, where $D_i = \{d|c_i\in d, d \in D_q\}$. $d(c_i, c_j) = 0$ when $D_i = D_j$, i.e., when $c_i$ and $c_j$ always co-occur in retrieved documents and are therefore very close semantically. Therefore, even if two concepts $c_i, c_j$ frequently co-occur ($|D_i \cap D_j|$ is large), their distance is still far if their union is much larger than their intersection. This avoids the problem where a concept is viewed to be close to many other concepts simply because it appears in many documents (e.g., concepts in the query that are prevalent in search results).

% based on the pair-wise distance of all the selected concepts, where each concept starts in its own cluster, and the pair of clusters with the smallest distance are merged at each step. Given two concepts $c_i$ and $c_j$ and two sets of documents $D_i$ and $D_j$ where the two concepts are mentioned respectively, the distance between the two concepts is calculated as $|D_i| + |D_j| - 2|D_i \cap D_j|$, so that high co-occurrence frequency results in small distance. We used the distance between the farthest points of two clusters as their distance measure.

The hierarchical clustering algorithm produced a tree structure where each leaf corresponds to a concept. To generate partitions, we cut the tree such that each  sub-tree is as large as possible but has no more than one-third of all concepts (leaf nodes) in the original tree. This method is able to produce partitions with relatively balanced sizes regardless of the original tree structure.  This approach is different from the commonly used method of cutting the tree at a fixed level, which may produce one very large partition or numerous small partitions if the original tree structure is highly skewed. Figure \ref{fig:graph_partitioning} illustrates a concrete example of our partitioning method. 

\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/dendro.drawio.png}
\Description[Graph partitioning]{Graph partitioning}
\caption{(a) The hierarchical clustering algorithm produced a tree structure. (b) Cutting the hierarchy at a fixed distance level can easily generate one very large partition (A) or numerous small partitions (B). (c) We cut the tree such that each sub-tree is as large as possible but has no more than one third of all leaf nodes. (d) Cluster A is a valid cluster as including one more node will result in a cluster (cluster B) with seven nodes, exceeding one third of the total number of leaf nodes (20 nodes in total).}
\label{fig:graph_partitioning}
\end{figure}


% An intuitive method of grouping concepts into clusters is to cut the tree at a set distance level to achieve the desired number of clusters or to restrict the max distance within a cluster. This method may produce very large or very small clusters for a skewed tree, which is not informative either way. We instead controlled the size of each cluster and cut the concept tree into sub-trees with less than a third of the total number of leaves. This method ensures that users are presented with concept clusters of reasonable size no matter what the tree structure looks like.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Graphical Faceted Search Interface}

The data model described in the previous section provides input to the frontend interface of GRAFS.
In this section, we first present our design goals for GRAFS, and then describe our implementation of the search interface.

\subsubsection{Design Goals}
Informed by the challenges of exploratory search described earlier in this paper, we propose the following design goals for the interactive experience enabled by GRAFS.
% We designed GRAFS to improve user's exploration and learning experience on a large searching result space. Consider the case of biomedical literature review, where users are presented with a few thousand articles retrieved by a search query. To make sense of the large information space, users still need to spend the majority of their time on reading articles. However, presented with the large set of articles, it can be challenging to learn an overview of the topic within a short time. That's where the data model, including the per-query knowledge graph, per-query concept grounding, and per-query concept clustering, can help. GRAFS was designed to incorporate the summarizing information generated by our data model as visual hint to help user explore through the information space and construct a conceptual understanding of the topic efficiently. With those tasks in mind, we identified three key design requirements: 
\begin{itemize}
    \item [\textbf{DG1}] \textbf{Preserve the simplicity, familiarity, and capability of a search interface.} Search engine users are well educated to use Google-like list presentation and faceted navigation interface. We aim to maintain the usability of the new search interface by leveraging the basic layout and functionality of existing systems.
    \item [\textbf{DG2}] \textbf{Show relations between concepts without cluttering the interface.}  Visualizing relations between concepts  has great potential to help users explore the information space. However, high-density connections can easily clutter the interface and discourage learning. We aim to selectively expose these relations in a sparse, non-cluttering manner.
    \item [\textbf{DG3}] \textbf{Preserve human agency.} The generated initial knowledge subgraph is meant to initiate the user's learning activities. 
    Users should have the ability to make adjustments to the knowledge subgraph based on their mental model or current interest during the sensemaking process.
    % The interface should allow users to make adjustments to the machine-generated concept list, which may not always make sense. Human correction and feedback can incorporate people's knowledge into the system and reflect current interest, which provides better exploration experience for users.
\end{itemize}
% The major space is still the ranked list of document. GRAFS should support basic search engine functions such as constructing queries, browsing multiple pages of the results, and read individual articles.

% Help users see connections between concepts in search. 

% Allow users to make adjustments. Domain experts working on biomedical literature review mentioned that machine-generated groupings of terms or concepts (topic models) in current available tools may not always make sense. 

\subsubsection{Implementation}

\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/action_view.png}
\Description[Initial view]{Initial view}
\caption{GRAFS for the topic ``treatment for depression'', including (A) the \textbf{graphical facet list} containing key concepts and their relations represented by arcs, (B) the \textbf{graphical facet treemap} showing the hierarchical structure of concepts based on the graph partitioning results, (C) the \textbf{document list} showing filtered articles ranked by their relevance to the search query, (D) the \textbf{concept provenance} that lists three examples of the selected concept. }
\label{fig:action_view}
\end{figure}

We implement GRAFS as an interactive web application. Its frontend elements leverage the JavaScript library D3.js. Its backend document indexing and search functions are based on Apache Solr.
At the beginning of a search,  a user can issue her search query of interest in the same manner as in a typical search engine. Simple keyword queries or complex Boolean queries are supported.  The user can also specify the number of documents ($|D_q|$) to retrieve (which by default is set to 1,000). 
After retrieving a set of documents, the system backend will compute the data model (knowledge subgraph, concept provenance, and graph partitioning) on the fly, which will serve as the input to the frontend interface. The user can specify the desired number of concepts in the knowledge subgraph (which by default is set to 20).

% In addition, the system allows the user to modify the desired number of concepts in the initial KG to show (which by default is set to 20).  
% back-end of our system will retrieve a set of relevant articles and compute the data model on the fly. The retrieved document set and the computed per-query KG, concept provenance, and graph partitioning will serve as the input of the user interface. 


\textbf{Interface Overview}.
A demonstration video showing all features of the GRAFS interface is \href{https://drive.google.com/file/d/1T36r-XxDQ8Y31AD1JFe6yUqtla_qvtR0/view?usp=sharing}{available online}.
Figure \ref{fig:action_view} shows the interface rendered for the search topic ``treatment for depression'' with 20 selected concepts.
To support exploratory search, GRAFS user interface (UI) follows the structure of a faceted search interface with a \textit{facet list} (Figure \ref{fig:action_view}(A)) on the left and a \textit{document list} (Figure \ref{fig:action_view}(C)) in the middle (\textbf{DG1}). In Figure \ref{fig:action_view}(A), each facet is a concept/node of the initial knowledge subgraph, which allows users to learn major concepts and filter articles by those concepts. The \textit{facet treemap} (Figure \ref{fig:action_view}(B)) shows a space-filling treemap~\cite{shneiderman1992tree} of  concepts, which visualizes the prevalence and relationship with each other. Given a selected concept (``Therapy'' in Figure \ref{fig:action_view}), the concept provenance sentences are listed on the right (Figure \ref{fig:action_view}(D)), providing a succinct summary of the concept.



% \subsubsection{1D graphical facets: facet list}

\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/concept_list_v2.pdf}
\Description[Initial view]{Initial view}
\caption{Facet list transitions. (a) The user starts with an initial view. (b) After the concept ``Therapy'' is selected, it is moved to the top of the facet list. Arcs are drawn to connect the selected concept to the five most related concepts. The arcs have the same color as the selected concept. (c) A second concept ``Clinical Trials'' is selected, and it is also moved to the top of the facet list. Relations between the intersection of the selected two concepts (at the top) and the other concepts are again shown by arcs. The arcs are grey when more than one concept is selected.}
\label{fig:concept_list}
\end{figure}

\textbf{1D Graphical Facet: Facet List}.
Figure \ref{fig:concept_list}(A) shows an initial view of the facet list.
The one-dimensional facet list contains the concepts/nodes in the knowledge subgraph. Based on the result of graph partitioning, the order of concepts follows the  order of leaves given by the cluster hierarchy and the color of each concept indicates its group identity. 


Users can select a concept to filter the retrieved document set so that only documents containing the select concept will be listed in the document list. For instance, the user might be interested in ``Therapy''. Upon selection, the concept (``Therapy'' in Figure \ref{fig:action_view} and \ref{fig:concept_list}(a)) will appear at the top of the list. The visualization component in the facet list was designed to facilitate users' exploration of the knowledge subgraph. To achieve this, arcs are drawn to connect the selected concept to the top five most related concepts in the knowledge subgraph. Those arc connections allow users to inspect a small portion of the per-query KG given current search focus and get a visual hint about possibly interesting concepts to explore on. As we define the relation between concepts to be their co-occurrence frequency, the five concepts co-occur most with ``Therapy'' are connected and the thickness of the arcs is proportional to the co-occurrence frequency. For instance, ``Therapy'', and its most frequently co-occurring concept ``Clinical Trials'' appear together in 50 documents.

% arc colors, hover behavior

The interface also allows users to further narrow down the search results by applying multiple filters. When more than one concept is selected, only documents that contain all the selected concepts will be included in the interface. For instance, the user may observe that ``Quality of Life'' was clustered into the same group as ``Therapy'', but their connection is not as strong as other concepts such as ``Clinical Trials''. To answer the question, the user applied ``Quality of Life'', which allows the user to examine the documents where the two concepts co-occur. Further reading helped the user find several articles that mention ``Quality of Life'' as an important secondary outcome for measuring effectiveness of ``Therapy''. The relation between the two selected concepts and the rest concepts are again shown by arcs, where the thickness indicates co-occurrence frequency, as shown in Figure \ref{fig:concept_list}(c). The user may infer that ``Symptoms of Depression'' and ``Anxiety'' might be other measures of the effectiveness of ``Therapy'', and these measurements may also be used in ``Clinical trials''. They can confirm their hypothesis by further selection and reading. Therefore, these arcs in the facet list visually nudge the user to narrowing down their interest by selecting the next concept.

% These arcs  in the facet list explicitly show relations between selected concept(s) and unselected ones. They visually nudge the user to narrowing down their interest by selecting the next concept. As such, these arcs encourage users to compose concepts and   
%  (\textbf{R2})

% \subsubsection{2D graphical facets: facet treemap}
\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/treemap.pdf}
\Description[Initial view]{Initial view}
\caption{Facet treemap transitions by doing the same sequence of actions as in Figure  \ref{fig:concept_list}. The user first select ``Therapy'' from the initial view (a). In (b), the dark bar in each rectangle shows the overlap with the selected concepts. The user continue to select ``Clinical Trials'', giving (c). }
\label{fig:treemap}
\end{figure}

\textbf{2D Graphical Facet: Facet Treemap}.
To provide a spatial overview of the selected concepts, the GRAFS UI also includes the facet treemap, which directly shows the hierarchical structure given by graph partitioning. Each rectangle represents a concept. The rectangles are colored to match concepts' group identities, and the size of the rectangle reflects the prevalence of the corresponding concept. Figure \ref{fig:treemap} illustrates the transition of the facet treemap through an example.

The facet treemap serves as another way to explore the concept relation. The position of concepts gives clues to the distance between concepts. In addition, when the user selects concepts, a histogram is included in each concept's rectangle to show the percentage of documents containing the selected concepts. For instance, Figure \ref{fig:treemap} (b) shows the facet treemap after selecting ``Therapy'', and the darker area in ``Clinical Trials'' shows the percentage of documents mentioning ``Therapy'' among all the documents containing ``Clinical Trials''. 

Different from the arc connections indicating the co-occurrence frequency, those percentage histograms reflect concept relations relative to concept prevalence (\textbf{DG2}). This property helps surface interesting relations that might be hidden by arcs, especially for less frequent concepts. For instance, after selecting ``Prophylactic treatment'', ``Postnatal depression'' appears to be closely relate to it in the facet treemap, and this relation seems to be stronger comparing to ``Symptoms of Depression''(Figure \ref{fig:prevent_treatment}). This relation can be easily ignored if the user only looks at the arcs as the connection of ``Prophylactic treatment'' with ``Symptoms of Depression'' seems to be much stronger than with ``Postnatal depression''.

\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/prevent_treatment.drawio.pdf}
\Description[prevent treatment]{prevent treatment}
\caption{The facet treemap may help surface interesting relations hidden by arcs. The strong relation between ``Prophylactic treatment'' and ``Postnatal depression'' shown in (a) is not obvious in (b).}
\label{fig:prevent_treatment}
\end{figure}

As the facet list and the facet treemap contains the same set of concepts, we use brushing techniques to synchronize interactions on either of them. Users can select a concept by directly clicking on it through the facet treemap, and the facet list will be re-rendered to incorporate the selection. Hovering over a concept on the facet treemap also has the same effects as hovering over the facet list.

\begin{figure}[t]
\centering  
\includegraphics[width=0.9\textwidth]{fig/edit_list.pdf}
\Description[edit]{edit}
\caption{Deletion can either be done through the facet list (a) or the facet treemap (b). The deleted concepts will be listed in the interface, and users may add them back as in (c). (d) Users can add recognized SNOMED concepts to the facet list from documents.}
\label{fig:edit_list}
\end{figure}

% \subsubsection{Editable list}
\textbf{Editable List}.
Users may want to make changes to the facet list based on their domain knowledge or new discoveries during their exploration. As shown in Figure \ref{fig:edit_list}, users can add new concepts or remove existing concepts from the list. Deletion can either be done through the facet list or the facet treemap. The deleted concepts will be listed separately in the interface in case the user wants to add the concept back. Users may encounter interesting concepts in articles during exploration and want to gain deeper understanding of them. To facilitate this, all the recognized SNOMED-CT concepts are annotated in articles and can be added to the facet list. The adding and removal of concepts will trigger the data model to re-calculate the knowledge subgraph and graph partitioning given the edited facet list (\textbf{DG3}). 

% \subsubsection{Concept provenance}
\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/example.pdf}
\Description[Initial view]{Initial view}
\caption{Concept provenance. In (a), as the user hover over a concept in facet list, the type of the concept and an example is shown in a tool-tip next to the concept. In (b), when the user select a concept, three examples are shown to provide a brief summary of how the concept is used in context.}
\label{fig:example}
\end{figure}

\textbf{Concept Provenance}.
Concept provenance sentences are included as (1) tooltip shown to the left of the facet list when the user hovers on a concept and (2) contextual examples listed on the right. The tooltip only includes the most related sentence extracted, aiming at providing a quick explanation of the concept as the user goes through the concept list. Users can refer to more use cases in contextual examples. Figure \ref{fig:example} shows concept provenance features.

\subsection{Baseline Faceted Search Interface}
\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/baseline.png}
\Description[Initial view]{Initial view}
\caption{Baseline search interface. It contains (A) \textbf{facet list} where concepts are organized by pre-defined categories, (B) \textbf{document list} showing filtered articles ranked by their relevance to the search query, (C) \textbf{concept provenance} that lists 3 examples of the selected concept.}
\label{fig:baseline}
\end{figure}
We compared GRAFS to a typical faceted search interface with a list of facets on the left and a ranked list of document taking the major part of the page as shown in Figure \ref{fig:baseline}. To minimize the difference in the information conveyed by the two systems, we applied the same concept selection method as in GRAFS. In the baseline system, however, concepts are organized by pre-defined categories. The knowledge subgraph and graph partitioning information are not surfaced in the baseline interface.

% \subsubsection{Overall search interface layout}

% 1. search results space is large

% 2. facet list is on the left side

% 3. visualization is not dominating the page

% \subsubsection{Graphical facets}

% 1. 1D presentation: facet list, explanations = tooltips, connections = arcs; groups = colors

% 2. 2D presentation: spatial relations. connections = distribution maps; groups = colors. 

% 3. when selecting one or multiple: ...




==> tex/motivation.tex <==
\section{Motivating Scenario and Current Tools}



As a motivating example for the challenges in designing search interfaces for presenting text-mined concepts to support exploratory search, consider the Thalia search engine~\cite{thalia}. Thalia uses natural language processing algorithms to extract UMLS concepts from all search results and use them as faceted filters. As shown in Figure \ref{fig:thalia}, the search query is ``treatment for depression'', and this results in an exceedingly long list of concepts in the faceted filter.

This situation happens because of two reasons. First, the UMLS Metathesaurus contains millions of concepts that cover a wide variety of domains in medicine. Second, natural language processing algorithms such as named entity recognition and linking aims to detect and map \emph{all} concepts mentioned in the full-text without missing any. As a result, these concepts will form a long-tail distribution in the search results: some concepts will appear with high frequency, and many concepts will appear with low frequency.

We observe three difficulties in Thalia's faceted search interface. First, the sheer number of concepts makes it overwhelming to present all of them.  Even though Thalia separated the long list of UMLS concepts into multiple facets (semantic categories defined by UMLS), there can still be hundreds of concepts under each category. A user needs to scroll multiple screens to see all of them. Second, top ranked concepts in each category are dominated by frequent yet non-informative concepts. For example, under the query ``treatment for depression'', the top-ranked concepts in each category are: oxygen in Chemical; tumor in Disease; alcohol in Drug, human in Gene/Species, glucose in Metabolite, cell in Anatomical. All these concepts frequently appear in many query, therefore not specifically attached to ``treatment for depression''. (This is reminiscent of ``stop words'' in information retrieval). These concepts may not help an exploratory learner build up context specifically for a query. Third, semantic categories are defined by an ontology, which is search context-agnostic. Such an organization of concepts does not easily reveal concept relations  \emph{within the context of the search}. To find out such relations, the user needs to memorize the ranking of concepts before selection, select a concept, and observe the change of relative ranking of concepts  after the selection. Such operations impose high demand on user's cognitive ability, creating a barrier for an exploratory searcher who is still learning about these concepts.

The above case study points at a few important considerations in designing a new faceted search interface to support the learning stage of an exploratory searcher. First, although the search results may be associated with many concepts, a search system can present a subset of relevant concepts for the user to get started in learning without being intimidated by the full complexity. Second, system-selected concepts may not be all useful, therefore the system may give users some control over what concepts to show and which to ignore. Third, the interface should encourage exploratory behavior by visual and interactive tools that makes relations easily visible. These considerations motivates our design of the graphical faceted search interface in the next section.







% \subsection{Semantic search engines with rich semantic annotation}

% \subsection{Challenges in Presenting Semantic Annotations to Support Exploratory Search}

% The rich semantic annotations are  useful in a variety of ways. In the backend of search engines, semantic annotations have long been used as internal representation of documents that enable queries to be matched with documents at a conceptual level, improving search performance.
% In the frontend, semantic annotations are increasingly used as interface elements visible to the user (Figure \ref{fig:current-tools}). They allow users to specify their information needs in an unambiguous manner as search terms or filtering constraints (Figure \ref{fig:current-tools}a). 
% They can also afford useful navigational features to help exploratory search tasks. For example, semantic concepts can be used as faceted filters to give an overview of the search results and enable multi-faceted filtering and query preview during exploratory search (Figure \ref{fig:current-tools}b), and create search result visualizations (Figure \ref{fig:current-tools}c).




% In an exploratory search task, a searcher is often motivated by a complex information problem, begins with a poor understanding of the terminology and the information space structure yet a strong desire to learn~\cite{white-supporting-exploratory-search}. Naturally, a user often starts the search process by trying to make sense of the complex information space, including recognizing important concepts, understanding their relevance in the context of search, and  discovering relationships between concepts. By gradually understanding of the information space, a user will be able navigate the space in an informed manner, e.g. by focusing on specific aspects of the information space and read into associated results. 

% To help searchers with such a task, many search systems -- especially literature search systems --  present semantic annotations along with search results. However, having a large vocabulary of semantic concepts brings a series of challenges when presenting them in a search interface.



% First, users may not be familiar with the search example


% 1. It helps to know key concepts in the search space, but the concepts are too many and unfamiliar to the user. Their relations are also unclear in the context of the current search.

% If we do not show (at least part) ontology (i.e. the PubMed way), then the user loses the chance to explore, learn, and refine the search scope.

% 2. If we show concepts in ontology in the interface, then the ontology is huge and we can only afford to show a small number of relevant ones. Those effectively become the facet-values in a faceted search interface, then the facet list can only contain ~20 concepts. This means we can only show a small subset of all concepts in the search results. 



==> tex/results_v1.tex <==
\section{Results}

% show only data in the results

% put the discussion/interprtation/take-aways into discussion
% address the tension between complexity and easy-to-use
Overall, the results from our study support \textbf{Hypothesis 1.a} and \textbf{Hypothesis 2}. We observed less clear results for \textbf{Hypothesis 1.b}. Though there is some evidence supporting \textbf{Hypothesis 1.b}, our study also illustrates certain challenges in confirming the effects of different systems on exploratory tasks. This section presents the results and feedback obtained from our study, and a number of insights uncovered during our analysis.

\subsection{Overview}
\label{sec:result overview}
The presentation of the study's results and our key observations are organized according to the hypotheses defined in Section \ref{sec:Hypotheses}. This overview provides a brief summary of the main findings, with more details provided in the remainder of this section.

\textbf{Hypothesis 1.} With the help of the knowledge subgraph, GRAFS positive influences users' conceptual understanding and sensemaking activities. 

\begin{itemize}
    \item [\textbf{1.a}] We found that GRAFS made it easier for users to see the relations between concepts (Q2) (Section \ref{sec:User Perceptions}, \ref{sec:Benefits of GRAFS and baseline})
    \item [\textbf{1.b}] We received mixed results for Hypothesis 1.b. The objective evaluation of user-generated outlines showed that participants were able to generate outlines with more depth (A3) when using GRAFS, supporting our hypothesis (Section \ref{sec:Outline Task}). Subjectively, meanwhile, a majority of participants preferred to use GRAFS for the given tasks (I4), indicating that GRAFS facilitated participants sensemaking activity. This also supports the hypothesis. However, no difference was observed for the overall quality of user-generated outlines (A6) across the two systems, and participants did not indicate in the questionnaire (Q1, Q3, Q4) that GRAFS helped them develop deeper understanding of the search topic (Section \ref{sec:User Perceptions}, \ref{sec:Outline Task}). Our results also showed that the baseline system helped participants collect more documents (A4) to support their arguments, and more participants believed the outlines they generated using the baseline is better (I1) ( Section \ref{sec:Outline Task}, \ref{sec:Evaluation of Generated Outlines}).
\end{itemize}
\textbf{Hypothesis 2.} The additional complexity introduced in GRAFS has no negative influence on users' searching activity.
\begin{itemize}
    \item [\textbf{2.a}] We found GRAFS did not make it more difficult to do the facet filtering task evaluated subjectively by participants (Q5) (Section \ref{sec:User Perceptions}) and objectively by the time participants spend on the facet filtering task (Section \ref{sec:Question-Answering Task}).
    \item [\textbf{2.b}] We found GRAFS was rated similar to the baseline system on the usability metrics (Q6 - Q9) (Section \ref{sec:User Perceptions}). GRAFS is more stimulating (Q8) and less manageable (Q7) than the baseline system (marginally significant). The majority of participants (14 out of 20) selected GRAFS for the future task (I4) (Section \ref{sec:User Perceptions}). Overall, participants provided positive feedback for the newly introduced components (I3, I4) (Section \ref{sec:Benefits of GRAFS and baseline}, \ref{sec:Usability of interface features}). However, the \textit{concept treemap} and the function of deleting and adding concepts were both more beneficial for users with relatively deeper understanding of the topic compared to \textit{concept arcs} and \textit{concept example tooltips}. 
\end{itemize}


% \begin{itemize}
%     \item Help users see the relation between concepts. Overall, still easy to use and manageable.
%     \item Effects on exploratory search:  stimulating, deeper understanding, interaction with the data model
%     \item Most useful and appreciated components
%     \item Overall prefers our system
%     \item Complexity or challenges
% \end{itemize}
\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/result.pdf}
\Description[result1]{result1}
\caption{Results. (a) Mean ratings given by participants in the post-task questionnaire. Error bars show the standard error. There is a significant difference between GRAFS and the baseline in Q2 (**), a marginally significant difference in Q7 and Q8 (*). (b) Numbers of votes given to each system by graders (A1-A6) and participants (I1, I4). GRAFS gets more votes in A3 depth and I4 system preference, while the baseline gets more votes in A4 documentation and I1 self-grading. Overall, there is no difference between the outlines generated using the two systems (A6).}
\label{fig:res1}
\end{figure}

\subsection{User Perceptions}
\label{sec:User Perceptions}
We evaluated participants' perception of the system through the ratings provided in the post-task questionnaire. Every participant provided two sets of ratings, one for each system. The mean overall ratings provided for each system are shown in Figure \ref{fig:res1}(a). The error bars show the standard error. We used Fisher's Randomization test to see whether the ratings given to the two systems are significantly different from each other. 

As shown in Figure \ref{fig:res1}(a), participants thought the two systems were different in helping them see the relation between concepts ($Avg_{GRAFS}=6.0$, $Avg_{Baseline}=5.0$, $p < 0.05$). This provides support for \textbf{Hypothesis 1.a} that GRAFS helps users see the relations between concepts better.

In contrast, the search system did not have significant effects on questions related to Q1 overview, Q3 discover, and Q4 decision. These results failed to show evidence supporting the \textbf{Hypothesis 1.b}.

The questionnaire results generally support \textbf{Hypothesis 2}. There is no significant difference in Q5, indicating that the additional features in GRAFS did not make the facet filtering task more difficult (\textbf{Hypothesis 2.a}). The system usability questions (Q6-Q9) provide supporting evidence for \textbf{Hypothesis 2.b}. There is no significant difference in Q6 Easy to use and Q9 Well-organized, while the differences in Q7 Manageable ($Avg_{GRAFS}=5.5$, $Avg_{Baseline}=6.0$, $p < 0.1$) and Q8 Stimulating ($Avg_{GRAFS}=5.95$, $Avg_{Baseline}=5.45$, $p < 0.1$) are only marginally significant. 

% task 2, easy to use, and organized. However, participants did think the two systems were different in helping them see the relation between concepts ($M_{GRAFS}=6.0$, $M_{Baseline}=5.0$, $p < 0.05$) (RQ2). Participants also perceived the Baseline system as being more manageable (RQ5) ($M_{GRAFS}=5.5$, $M_{Baseline}=6.0$, $p < 0.1$) and GRAFS as being more stimulating ($M_{GRAFS}=5.95$, $M_{Baseline}=5.45$, $p < 0.1$) (RQ3).


\subsection{Outline Task}
\label{sec:Outline Task}
% Need to provide an example

Figure \ref{fig:res1} (b) shows graders' votes for the two systems (A1-A6), participants' self-grading of their summaries (I1), and participants' system preferences (I4). Overall, there are some evidence supporting \textbf{Hypothesis 1.b}, but we also found multiple factors that make it difficult to evaluate the influence of different systems on participants' performance.

For the depth of the outline (A4), graders gave 12 votes to GRAFS and 8 to the baseline, supporting \textbf{Hypothesis 1.b}. In terms of documentation (A2), 12 votes went to the baseline system and 8 went to GRAFS, indicating that being exposed to relation information may have negative effects on people's searching or foraging behavior. When using GRAFS, participants may spend more time on exploring concept relations and developing deeper understanding, with less time left for collecting supporting documents. GRAFS and the baseline system received the same or similar number of votes in structure, interpretation, diversity, and overall quality. Overall, only A4 supports \textbf{Hypothesis 1.b} and the remaining criteria disagree with it in terms of the objective evaluation of outlines. 

During exit interview, We found that  topic difference and participants' background may have bigger impact on outline quality than the system. For instance, five participants mentioned that they were more familiar with one of the topics, and those participants felt that they did a better job on the familiar topic. We provide more details in Section \ref{sec:Evaluation of Generated Outlines}. One the one hand,those factors may influence the comparison of the number of votes given to each system due to the small sample size we have. On the other hand, those factors may cover the system difference (e.g. if participants always perform better on one topic, then GRAFS and Baseline will always get equal votes).

% For structure, interpretation, diversity, and overall quality, GRAFS and the baseline system received the same or similar number of votes. In terms of documentation, 12 votes went to the baseline system and 8 went to GRAFS. For the depth of the outline, graders gave 12 votes to GRAFS and 8 to the baseline. Based on the external grading, GRAFS supported participants to generate deeper outlines (RQ3), while the baseline system can help participants find more supporting documents (RQ5). However, for most of the quality measures, including the overall quality, the outlines generated through the two systems didn't have large deviation. We hypothesize that other factors such as background or experience may have bigger impact on outline quality. We provide more detailed discussion in section 5.4.2 based on feedback collected during the exit interview.

When evaluating the generated outlines, a majority of the participants felt that they did a better job producing their outlines using the baseline system (I1). Interestingly, when asked which system they would use if they were to do the task again, the majority of the participants selected GRAFS (I4). Combining with questionnaire responses, one possible explanation is that being exposed to concept relations (Q2) increase complexity such that the user interface becomes less manageable (Q7). However, participants still found that relation information was useful for the exploratory task. Therefore, users expressed a preferences for GRAFS because, if given more time on task, it would support a  deeper understanding of the topic during exploratory literature search. In this way, participants' preference for GRAFS can be viewed as evidence for \textbf{Hypothesis 1}.

% This illustrates that participants prefer GRAFS for exploratory search, but GRAFS may not necessarily help with the outcome of the task. We seek to further understand this phenomenon through interview analysis in section 5.4.1 and 5.4.2.

\subsection{Question-Answering Task}
\label{sec:Question-Answering Task}
Participants indicated their perception of the difficulty of the question answering task through the post-task questionnaire. As mentioned in Section \ref{sec:result overview}, there is no significant difference between the ratings given to the two systems regarding the task's difficulty. We further evaluated participants' performance based on the time spent on the task. On average, participants spent 181.1s on question answering task using GRAFS and 238.2s using the baseline system, and the difference is not significant. This shows that participants performed the lookup task at least as well on GRAFS as on a typical faceted search system, which supports \textbf{Hypothesis 2.a}.


\subsection{Qualitative User Feedback}
\label{sec:Qualitative User Feedback}

\subsubsection{Benefits of GRAFS and Baseline}
\label{sec:Benefits of GRAFS and baseline}
% May give some examples for each of the feedback mentioned 

As mentioned in Section \ref{sec:result overview}, the majority of participants preferred GRAFS over the baseline system (14:6). During the exit interview, we asked participants to indicate the reason of their preference. In general, participants' feedback shows that the new information and functions provided by GRAFS facilitated users' exploratory activity, while introducing some complexity to the system. 

Participants described benefits of GRAFS related to: (1) relations, (2) specific components, and (3) general experience. Several users ($n=4$) mentioned that they loved the fact that they can learn relations between concepts in GRAFS (\textbf{Hypothesis 1.a}). Many participants ($n=7$) mentioned some components that they particularly liked, including facet treemap ($n=4$), editable list ($n=3$), and facet list arcs ($n=3$). Four participants selected GRAFS for a better overall experience. Specifically, they mentioned GRAFS is interesting and colorful ($n=2$), and helps with overview ($n=1$) and new ideas ($n=1$). These comments reflect that a majority of the participants found the newly introduced components usable and were able to apply those new information into their tasks, providing support for \textbf{Hypothesis 2.b}.

Most of the participants that preferred the baseline system thought the baseline system is clearer ($n=4$), while two mentioned that they liked the pre-defined categories ($n=2$).
% For instance, User 2 said that she preferred GRAFS mainly because she can edit the concept list in this system.

\subsubsection{Evaluation of Generated Outlines}
\label{sec:Evaluation of Generated Outlines}
% While most of the participants appreciated the new information and function provided in GRAFS, we didn't observe major difference in the quality of people's outlines except for documentation and depth. When asked which outline they preferred, most of the participants selected the outline generated using the baseline system (baseline: 12, GRAFS: 7, no difference: 1). 
While most of the participants appreciated the new information and functions provided in GRAFS (I4), we did not observe major differences in the quality of people's outlines except in the aspects of documentation and depth. Participants' comments indicate that the interface design did effect their activity when completing the task, but the influence of search topic on a user's outline proved to be larger in our analysis.
% Therefore, \textbf{Hypothesis 1.b} might be very difficult to test.
 
Reflecting this, most of the participants ($n=12$) mentioned the influence of topic difference on the outline quality, including difficulty, familiarity, new vs old, and certainty of the results. Some participants ($n=6$) thought ``Treatment for Depression'' was easier than ``COVID-19 Diagnosis'' in terms of vocabulary and the topic's structure. Five participants mentioned that they were more familiar with one of the topics, and those participants felt that they did a better job on the familiar topic. Some participants ($n=4$) mentioned that the two topics were different from each other in the work required to perform the task, which in turn influenced the quality of the final outcomes. Three out of the four participants commented that they found depression to be a well-established field while COVID-19 related research was newer (and therefore harder to approach due to the more scattered and heterogeneous set of related concepts).
% For instance, User 12 mentioned that he had a better idea of how to approach the topic of depression, while the covid topic has a lot of new concepts and he didn't know how to start.

% As described by User 16, "For depression, there are much more evidence, studies, and clinical trials." Therefore, she was able to read more articles with more "systematic and analytical results" and saw the comparison between different treatment methods. But for COVID-19, "most of the articles only present simple findings". Therefore, her outline of covid was more like a simple list of methods she found. 

A number of participants ($n=6$) mentioned that the features of the interface affected the quality of their outline. Four users said that GRAFS helped them generate good summaries as it enabled them to edit the concept list ($n=2$), see relations between concepts ($n=1$), and was easier to use ($n=1$). In contrast, one participant thought the features in GRAFS were distracting and negatively influenced his work. One participant liked the categories given in the baseline system and helped her to write good summary. 

% Other feedback is related to task familiarity, and participants felt their second summary is better than the first one as they are more familiar with the task and how to approach it. This illustrates the necessity of counter-balancing the order of using the two systems.

% The disagreement between participants' preference of the system, self-grading of outlines' quality, and objective grading may be a mixed effects of search topics, interface designs, orders of doing the task, and background. As we only have 20 participants, it's hard to test those effects.

\subsubsection{Usability of Interface Features}
\label{sec:Usability of interface features}
%This section reports on the feedback collected focusing on each components we introduced in GRAFS to further test \textbf{Hypothesis 2.b}. 

During the exit interview, participants were asked whether a component is useful or not for accomplishing the given tasks.  We note that there is a difference between (1) a participant not using a feature, and (2) a participant finding the feature not useful after using it. More specifically, we noticed that some participants did not use certain features in GRAFS due to time limitation, lack of domain knowledge, and limited experience with a new interface design.
Therefore, we report both (1) the number of participants that used each feature based on the action log, and (2) the number of participants that found each feature to be useful. 

Overall, the facet list arcs were the most used feature. The facet treemap was used less often, in part due to its higher complexity. The functions of deleting and adding concepts were used least, reflecting that they require a deeper understanding of the topic and that they become most useful later in a task. Though these all add compelxity to the traditional faceted list search interface, the components all received positive feedback from participants. The concept provenance tooltip was found to be easy to use, but not as useful as other components.
% We focus on \textit{concept arcs}, \textit{concept treemap}, \textit{concept grounding examples}, \textit{editable list}.
% An overview of the use of components is show in table \ref{tab:components}.

% \begin{table}[H]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          \hline
%                                                                     & Useful & Not Useful & No Indication \\ \hline
% Concept Arcs                                                        & 11     & 9          & 0             \\ \hline
% Concept Treemap                                                     & 9      & 11         & 0             \\ \hline
% \begin{tabular}[c]{@{}c@{}}Concept Grounding\\ Tooltip\end{tabular} & 8      & 11         & 1             \\ \hline
% \begin{tabular}[c]{@{}c@{}}Editable List\\ Delete\end{tabular}      & 6      & 13         & 1             \\ \hline
% \begin{tabular}[c]{@{}c@{}}Editable List\\ Add\end{tabular}         & 4      & 15         & 1             \\ \hline
%     \end{tabular}
%     \caption{Use of components}
%     \label{tab:components}
% \end{table}

\textbf{Facet List Arcs:} Action logs show that all 20 participants made at least one selection from the facet list, which triggers the display of facet list arcs. The majority of participants thought the feature of concept arcs to be useful ($n=11$). Some participants ($n=6$) mentioned that arcs helped inform them about what to look at or which concepts to click next (\textbf{Hypothesis 1.b}). Five participants mentioned that arcs helped them understand relations between concepts (\textbf{Hypothesis 1.a}), which in turn helped them better understand the topic and adjust their selection strategy (\textbf{Hypothesis 1.b}). 
%Overall, these findings suggest that arcs encouraged participants' exploration and facilitated their understanding of the relations between concepts.

% For instance, User 7 said that he is not familiar with the topic, so the arcs helped him "see the basic idea of the topic and see what to pay attention to" and it’s "especially helpful during the initial exploration". One possible drawback mentioned by one of the participants is that arcs were repeatedly drawn between some concepts. Though the participant already examined that relation, her attention were still attracted to it, which is distracting. 

For participants that did not state that arcs were useful, a majority of them said that they ignored this feature ($n=5$). For instance, User 4 said that he preferred to just read articles and User 12 mentioned that due to time limitations, he was not able to use that information. Some participants ($n=2$) used alternatives to the arcs to get similar information, such as the facet treemap, or the number of documents listed near each concept.

\textbf{Facet Treemap:} We considered a participant to have used the facet treemap if they clicked at least once on a concept in the visualization, or if they hovered the mouse over any concept in the facet treemap for more than one second. All of the participants meet this criterion. Nine out of 20 participants thought facet treemap to be useful. Participant feedback illustrates that the facet treemap can be difficult to make sense of due to its unfamiliarity, and it introduces complexity to using the system. Yet while it may take time for users to learn how to use this feature, nine out of 20 participants thought that the facet treemap was useful. 

Most of the participants who found it useful ($n=8$) reported that the facet treemap helped them see the relations between concepts (\textbf{Hypothesis 1.a}). Because both the facet treemap and the facet list arcs communicate the connections between concepts, some participants ($n=7$) compared the two. Five participants indicated that they preferred facet treemap compared to facet list arcs, while the other two participants preferred arcs. Those two felt that the arcs were more straightforward. 

Interestingly, among people that preferred the facet treemap, two participants commented that facet treemap was not straightforward to understand and that it took time for them to find it useful. For instance, User 20 mentioned that he didn’t find treemap to be useful immediately. However, during the exploration, he found that thick arcs in the facet list always seemed to connect to broader concepts such as infectious disease. He therefore started to look to the treemap for a more nuanced view of the relations and, eventually, found the treemap to be more useful.

% Some participants (n=2) also found that treemap is easy to click and good for navigation. One participants thought treemap can provide an overview of the topic.

A majority of the participants ($n=11$) did not report the facet treemap as being useful. Three participants felt the information was cluttered and overwhelming, while some participants ($n=2$) thought it occupied too much screen space. Three participants mentioned that it was difficult to make sense of the information provided by the facet treemap, and two participants said they were not used to information presented in that way. Many of these comments suggest unfamiliarity as a key hurdle.

\textbf{Concept Provenance:} All participants used this feature when hovering over items in the facet list. Eight participants mentioned that the facet list tooltip was useful. Some participants ($n=4$) mentioned that the tooltip helped them gain a quick understanding of what the concept meant. Two participants expressed the wish that they could navigate directly to an original article from the given examples. 

For people that did not report that the facet list tooltip was useful, four mentioned that they did not need extra explanations of the concepts either because they had good background knowledge or they only used familiar concepts during their exploration. Some participants ($n=3$) preferred to understand concepts using other method, such as ``googling'' or reading the actual articles. One participant mentioned that the usefulness of the tooltip was highly dependent on its quality. Overall, the concept provenance tooltips were found to help people understand concepts during exploration, but only when users were faced with new concepts.
% During the exit interview, we focused on the concept grounding tooltip shown next to the concept list. 

\textbf{Editable List:} GRAFS allows users to make adjustments to the automatically generated knowledge subgraph by deleting or adding concepts. Overall, this feature was less used by participants due to task time  constraints, limited familiarity with the topic, and limited training with this way of interacting. However, participants provided positive feedback on this feature, and we found some interesting use cases that indicate the benefits of preserving human agency in GRAFS.

As most of the participants only used one part of the function (either add or delete, but not both), we examine the feedback regarding deleting concepts and adding concepts separately. Six of the 20 participants used the function of deleting concepts, and six participants mentioned that the function of deleting concepts was useful for removing irrelevant or equivalent variants of concepts. This helped users focus on a shortened concept list ($n=2$) and find important relations faster ($n=1$). 

Five of the 20 participants used the function of adding concepts, and four participants found adding concepts to be useful. Two people used this function when they came across unlisted concepts that they felt were important based on their reading. An interesting use case was provided by User 2. She described that when she worked on ``Treatment for Depression,'' she frequently came across the concept of ``Exercise.'' Therefore, she added ``Exercise'' to the concept list to investigate deeper. When she felt she had done enough reading of related materials, she then removed the concept from the list. One participant added the concept ``COVID-19,'' which was removed as a per-query stopword, to remind herself about the major topic. One participant suggested the interface should enable users to add new concepts to the facet list by directly typing in concept names in addition to selecting concepts in documents.

For participants that did not use the add or remove functions, four participants mentioned that time limitation was a major reason. Some participants ($n=3$) mentioned that the lack of familiarity with the topic is another important factor. 

% For instance, User 10 said that he "likes the fact that he can add new concepts into the concept list", though he didn’t use that function during the study, he "can imagine using that function if I spend a whole day to write the summary." 
% For instance, User 9 mentioned that she was not familiar with the concepts. But if she knew what she wanted, she "will be able to delete some concepts to shorten the list and be more focused." Besides, another two participants suggested that they wanted to customize concepts to add into the list.

\subsection{Additional Analysis}
% further analysis
\subsubsection{Influential Factors}
People's perceptions of the both GRAFS and the baseline faceted search system may vary with their background and the order of using the systems. In our analysis, we split participants into groups considering the order of using the two systems ($G_{order}$), whether they have biomedical domain knowledge ($G_{domain}$), experience of conducting a literature review ($G_{experience}$), and topic familiarity ($G_{familiar}$). We evaluated the effects of these group identities on the questionnaire responses that had statistically significant findings (Q2 relation, Q7 manageable, and Q8 stimulating) with a mixed ANOVA model. The group identities were treated as between-subject factors and the system (GRAFS or baseline) was treated as a within-subject factor. 
\begin{table}[h]
\begin{tabular}{llll}
\hline
                    & F     & $\eta^2$ & p     \\ \hline
$G_{order}$        & 0.323 & 0.018  & 0.577 \\ 
$System$              & 6.406 & 0.262  & 0.021 \\ 
$G_{order}\times System$ & 3.139 & 0.148  & 0.093 \\ \hline
\end{tabular}
\caption{Effect of order on user's rating of relation}
\end{table}

\begin{table}[h]
\begin{tabular}{llll}
\hline
                    & F     & $\eta^2$ & p     \\ \hline
$G_{domain}$       & 6.170 & 0.255  & 0.023 \\ 
$System$              & 1.797 & 0.091  & 0.197 \\ 
$G_{domain}\times System$ & 0.002 & 0.000  & 0.967 \\ \hline
\end{tabular}
\caption{Effect of domain knowledge on user's rating of easy to use}
\end{table}

\begin{table}[h]
\begin{tabular}{llll}
\hline
                    & F     & $\eta^2$ & p     \\ \hline
$G_{domain}$       & 8.160 & 0.312  & 0.010 \\ 
$System$              & 3.635 & 0.168  & 0.073 \\ 
$G_{domain}\times System$ & 0.173 & 0.010  & 0.682 \\ \hline
\end{tabular}
\caption{Effect of domain knowledge on user's rating of manageable}
\end{table}

\begin{figure}[t]
\centering  
\includegraphics[width=1\textwidth]{fig/result_effect.pdf}
\Description[result1]{result1}
\caption{The effects of the order of using the two systems and participants' domain knowledge on participants' perception of the system. (a) Participants that worked on GRAFS first gave lower scores to the baseline in the system's ability to help them see the relation between concepts. (b) Biomedical domain experts gave higher scores to ``easy to use'' compared to participants without domain knowledge. (c) Biomedical domain experts gave higher scores to ``Manageable'' compared to participants without domain knowledge.}
\label{fig:res_effect}
\end{figure}

Topic familiarity and literature search experience did not have any effect on participants' ratings. A significant interaction effect between the order and system was found for participants' rating on the relation (p<0.1). As shown in figure \ref{fig:res_effect}(a), when rating whether the system helps to see concept relations, people that worked on GRAFS first tend to give lower scores to the baseline system compared to the case when the user started from the baseline system. This phenomenon indicates that users did use some of the provided visual representations in GRAFS to perceive the relations between concepts. When exposed to the baseline system as the second interface, users appeared to have an increased awareness of the difficulty in seeing concept relations without the GRAFS features. This further supports our \textbf{Hypothesis 1}. 
% (a table, post hoc?)
Additionally, participants with biomedical background gave significantly higher scores for the question of easy to use and manageable for both GRAFS and the baseline system. The effect of $G_{domain}$ is more significant than the effect of the system on the two questions. This shows that people's judgement of a system's usability is highly influenced by people's domain knowledge.

% \subsubsection{Compare concept selection behaviors of the two systems}





==> tex/results_v2.tex <==
\section{Results}

% show only data in the results

% put the discussion/interprtation/take-aways into discussion
% address the tension between complexity and easy-to-use
Overall, the results from our study support \textbf{Hypothesis 1.a} and \textbf{Hypothesis 2}. We observed less clear results for \textbf{Hypothesis 1.b}. Though there is some evidence supporting \textbf{Hypothesis 1.b}, our study also illustrates certain challenges in confirming the effects of different systems on exploratory tasks. This section presents the results and feedback obtained from our study, and a number of insights uncovered during our analysis. Fisher's randomization test was used to test for  significant effects due to  system difference~\cite{smucker2007comparison}. We interpret an effect as \emph{significant} if $p < .05$, and \emph{weakly significant} if $.05 \le p < .1$.

\subsection{Overview}
\label{sec:result overview}
The presentation of the study's results and our key observations are organized according to the hypotheses defined in Section \ref{sec:Hypotheses}. This overview provides a brief summary of the main findings, with more details provided in the remainder of this section.

\textbf{Hypothesis 1.} With the help of the knowledge subgraph, GRAFS positively influences users' conceptual understanding and sensemaking activities. 

\begin{itemize}
    \item [\textbf{1.a}] We found that GRAFS made it easier for users to see the relations between concepts (Q2) (Section \ref{sec:User Perceptions Main}, \ref{sec:Benefits of GRAFS and baseline})
    \item [\textbf{1.b}] We received mixed results for Hypothesis 1.b. The objective evaluation of user-generated outlines showed that participants were able to generate outlines with more depth (A3) when using GRAFS, supporting our hypothesis (Section \ref{sec:Outline Task objective}). Subjectively, meanwhile, a majority of participants preferred to use GRAFS for the given tasks (I4), indicating that GRAFS facilitated participants' sensemaking activity (Section \ref{sec:Outline Task subjective}). This also supports the hypothesis. However, no difference was observed for the overall quality of user-generated outlines (A6) across the two systems, and participants did not indicate in the questionnaire (Q1, Q3, Q4) that GRAFS helped them develop deeper understanding of the search topic (Section \ref{sec:User Perceptions Main}, \ref{sec:Outline Task objective}). Our results also showed that the baseline system helped participants collect more documents (A4) to support their arguments, and more participants believed the outlines they generated using the baseline is better (I1) ( Section \ref{sec:Outline Task objective}, \ref{sec:Outline Task subjective}).
\end{itemize}
\textbf{Hypothesis 2.} The additional complexity introduced in GRAFS has no negative influence on users' searching activity.
\begin{itemize}
    \item [\textbf{2.a}] We found GRAFS did not make it more difficult to do the question answering task evaluated subjectively by participants (Q5) (Section \ref{sec:User Perceptions Main}) and objectively by the time participants spent on the question answering task (Section \ref{sec:Question-Answering Task}).
    \item [\textbf{2.b}] We found GRAFS was rated similar to the baseline system on the usability metrics (Q6 - Q9) (Section \ref{sec:User Perceptions Main}). GRAFS is more stimulating (Q8) and less manageable (Q7) than the baseline system (weakly significant). The majority of participants (14 out of 20) selected GRAFS for the future task (I4) (Section \ref{sec:Outline Task subjective}). Overall, participants provided positive feedback for the newly introduced components (I3, I4) (Section \ref{sec:Benefits of GRAFS and baseline}, \ref{sec:Usability of interface features}). However, the \textit{concept treemap} and the function of deleting and adding concepts were both more beneficial for users with relatively deeper understanding of the topic compared to \textit{concept arcs} and \textit{concept example tooltips}. 
\end{itemize}


% \begin{itemize}
%     \item Help users see the relation between concepts. Overall, still easy to use and manageable.
%     \item Effects on exploratory search:  stimulating, deeper understanding, interaction with the data model
%     \item Most useful and appreciated components
%     \item Overall prefers our system
%     \item Complexity or challenges
% \end{itemize}
\begin{figure}[t]
\centering  
\begin{subfigure}{.48\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{fig/res_a.pdf}
    \caption{Post-task questionnaire results}\label{fig:res_a}
\end{subfigure}
    \hfill
\begin{subfigure}{.5\textwidth}
    \centering
    \includegraphics[width=1\textwidth]{fig/res_b.pdf}
    \caption{Outline generation task results}\label{fig:res_b}
\end{subfigure}
% \includegraphics[width=1\textwidth]{fig/result.pdf}
% \Description[result1]{result1}
\caption{Results. (a) Mean ratings given by participants in the post-task questionnaire. Error bars show the standard error. There is a significant difference between GRAFS and the baseline in Q2 (**), a weakly significant difference in Q7 and Q8 (*). (b) Numbers of votes given to each system by graders (A1-A6) and participants (I1, I4). GRAFS gets more votes in A3 Topical depth and I4 System preference, while the baseline gets more votes in A4 Documentation and I1 Self-grading. Overall, there is no difference between the outlines generated using the two systems (A6).}
\label{fig:res1}
\end{figure}

\subsection{User Perceptions}
\label{sec:User Perceptions}
\subsubsection{Main Results}
\label{sec:User Perceptions Main}
We evaluated participants' perception of the system through the ratings provided in the post-task questionnaire. Every participant provided two sets of ratings, one for each system. The mean overall ratings provided for each system are shown in Figure \ref{fig:res1}(a). The error bars show the standard error. 
% We used Fisher's Randomization test to see whether the ratings given to the two systems are significantly different from each other. 

As shown in Figure \ref{fig:res1}(a), participants thought the two systems were different in helping them see the relation between concepts ($Avg_{GRAFS}=6.0$, $Avg_{Baseline}=5.0$, $p = 0.033$). This provides support for \textbf{Hypothesis 1.a} that GRAFS helps users see the relations between concepts better.

In contrast, the search system did not have significant effects on questions related to Q1 overview, Q3 discover, and Q4 decision. These results failed to show evidence supporting \textbf{Hypothesis 1.b}.

The questionnaire results generally support \textbf{Hypothesis 2}. There is no significant difference in Q5, indicating that the additional features in GRAFS did not make the question answering task more difficult (\textbf{Hypothesis 2.a}). The system usability questions (Q6-Q9) provide supporting evidence for \textbf{Hypothesis 2.b}. There is no significant difference in Q6 Easy to use and Q9 Well-organized, while the differences in Q7 Manageable ($Avg_{GRAFS}=5.5$, $Avg_{Baseline}=6.0$, $p = 0.099$) and Q8 Stimulating ($Avg_{GRAFS}=5.95$, $Avg_{Baseline}=5.45$, $p = 0.092$) are only weakly significant. 

\subsubsection{Factors Affecting Users' Perceptions of the Systems}
People's perceptions of the both GRAFS and the baseline faceted can be influenced by a variety of factors including their prior experiences and the order of using the systems. In our analysis, we split participants into groups considering the order in which they used the two systems ($G_{order}$), whether they have biomedical domain knowledge ($G_{domain}$), their experience with conducting a literature review ($G_{experience}$), and topic familiarity ($G_{familiar}$). We evaluated the effects of these group identities on the questionnaire responses with a mixed ANOVA model. The group identities were treated as between-subject factors and the system (GRAFS or baseline) was treated as a within-subject factor. 
\begin{table}[h]
\begin{tabular}{llll}
\hline
                    & F     & $\eta^2$ & p     \\ \hline
$G_{order}$        & 0.323 & 0.018  & 0.577 \\ 
$System$              & 6.406 & 0.262  & 0.021 \\ 
$G_{order}\times System$ & 3.139 & 0.148  & 0.093 \\ \hline
\end{tabular}
\caption{Effect of order on a user's rating of Q2 Relation}
\label{tab:order_effect}
\end{table}

\begin{table}[h]
\begin{tabular}{llll}
\hline
                    & F     & $\eta^2$ & p     \\ \hline
$G_{domain}$       & 6.170 & 0.255  & 0.023 \\ 
$System$              & 1.797 & 0.091  & 0.197 \\ 
$G_{domain}\times System$ & 0.002 & 0.000  & 0.967 \\ \hline
\end{tabular}
\caption{Effect of domain knowledge on a user's rating of Q6 Easy to use}
\label{tab:knowledge_effect1}
\end{table}

\begin{table}[h]
\begin{tabular}{llll}
\hline
                    & F     & $\eta^2$ & p     \\ \hline
$G_{domain}$       & 8.160 & 0.312  & 0.010 \\ 
$System$              & 3.635 & 0.168  & 0.073 \\ 
$G_{domain}\times System$ & 0.173 & 0.010  & 0.682 \\ \hline
\end{tabular}
\caption{Effect of domain knowledge on a user's rating of Q7 Manageable}
\label{tab:knowledge_effect2}
\end{table}

\begin{figure}[t]
\centering  
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/order_effect.png}
    \caption{The effect of order on Q2 Relation}\label{fig:effect1}
\end{subfigure}
    \hfill
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/domain_effect_easy.png}
    \caption{The effect of domain knowledge on Q6 Easy to use}\label{fig:effect2}
\end{subfigure}
    \hfill
\begin{subfigure}{.32\textwidth}
    \centering
    \includegraphics[width=1\linewidth]{fig/domain_effect_manage.png}
    \caption{The effect of domain knowledge on Q7 Manageable}\label{fig:effect3}
\end{subfigure}
% \includegraphics[width=1\textwidth]{fig/result_effect.pdf}
% \Description[result1]{result1}
\caption{The effects of the order of using the two systems and participants' domain knowledge on participants' perception of the system. (a) Participants that worked on GRAFS first gave lower scores to the baseline in the system's ability to help them see the relation between concepts. (b) Biomedical domain experts gave higher scores to Q6 Easy to use compared to participants without domain knowledge. (c) Biomedical domain experts gave higher scores to Q7 Manageable compared to participants without domain knowledge.}
\label{fig:res_effect}
\end{figure}

Topic familiarity and literature search experience did not have any measurable effect on participants' ratings. A weakly significant interaction effect between the order and system was found for participants' rating on Q2 Relation ($p = 0.093$, Table \ref{tab:order_effect}). As shown in Figure \ref{fig:res_effect}(a), when rating whether the system helps to see concept relations, people that worked on GRAFS first tended to give lower scores to the baseline system compared to the case when the user started from the baseline system. This phenomenon suggests that users did use some of the provided visual representations in GRAFS to perceive the relations between concepts. When exposed to the baseline system as the second interface, users appeared to have an increased awareness of the difficulty in seeing concept relations without the GRAFS features. This further supports our \textbf{Hypothesis 1}.
% (a table, post hoc?)

Additionally, participants with biomedical background gave significantly higher scores for Q6 Easy to use ($p = 0.023$, Table \ref{tab:knowledge_effect1}, Figure \ref{fig:res_effect}(b)) and Q7 Manageable ($p = 0.010$, Table \ref{tab:knowledge_effect2}, Figure \ref{fig:res_effect}(c)) for both GRAFS and the baseline system. The effect of $G_{domain}$ is more significant than the effect of the system on the responses for these two questions. This suggests that people's judgement of a system's usability is highly influenced by people's domain knowledge. No significant effect was found between $G_{domain}$ and the responses on Q2 Relation ($p = 0.414$), indicating that GRAFS helps the participants see concept relations no matter whether they have domain knowledge or not.
% task 2, easy to use, and organized. However, participants did think the two systems were different in helping them see the relation between concepts ($M_{GRAFS}=6.0$, $M_{Baseline}=5.0$, $p < 0.05$) (RQ2). Participants also perceived the Baseline system as being more manageable (RQ5) ($M_{GRAFS}=5.5$, $M_{Baseline}=6.0$, $p < 0.1$) and GRAFS as being more stimulating ($M_{GRAFS}=5.95$, $M_{Baseline}=5.45$, $p < 0.1$) (RQ3).


\subsection{Outline Generation Task}
\label{sec:Outline Task}
% Need to provide an example

Figure \ref{fig:res1} (b) shows graders' votes for the two systems (A1-A6), participants' self-grading of their outlines (I1), and participants' system preferences (I4). Overall, there are some evidence supporting \textbf{Hypothesis 1.b}, but we also found multiple factors that make it difficult to evaluate the influence of different systems on participants' performance.

\subsubsection{Objective Evaluation of the Generated Outlines}
\label{sec:Outline Task objective}
For A3 Topical depth, graders gave 12 votes to GRAFS and 8 to the baseline, supporting \textbf{Hypothesis 1.b}. In terms of A4 Documentation, 12 votes went to the baseline system and 8 went to GRAFS, indicating that being exposed to relation information may have negative effects on people's searching or foraging behavior. Therefore, A4 fails to support \textbf{Hypothesis 1.b}. One possible explanation is that when using GRAFS, participants may spend more time on exploring concept relations and developing deeper understanding, with less time left for collecting supporting documents. GRAFS and the baseline system received the same or similar number of votes in A1 Structure, A2 Interpretation, A5 Topical diversity, and A6 Overall quality, which fails to support \textbf{Hypothesis 1.b}. Overall, A3 supports \textbf{Hypothesis 1.b} and the remaining criteria disagree with it in terms of the objective evaluation of outlines. 

\subsubsection{Participants' Self Evaluation of the Generated Outlines}
\label{sec:Outline Task subjective}


% For structure, interpretation, diversity, and overall quality, GRAFS and the baseline system received the same or similar number of votes. In terms of documentation, 12 votes went to the baseline system and 8 went to GRAFS. For the depth of the outline, graders gave 12 votes to GRAFS and 8 to the baseline. Based on the external grading, GRAFS supported participants to generate deeper outlines (RQ3), while the baseline system can help participants find more supporting documents (RQ5). However, for most of the quality measures, including the overall quality, the outlines generated through the two systems didn't have large deviation. We hypothesize that other factors such as background or experience may have bigger impact on outline quality. We provide more detailed discussion in section 5.4.2 based on feedback collected during the exit interview.

When evaluating the generated outlines, a majority of the participants ($n=12$) felt that they did a better job producing their outlines using the baseline system (I1). Interestingly, when asked which system they would use if they were to do the task again, the majority of the participants ($n=14$) selected GRAFS (I4). Combining with questionnaire responses, one possible explanation is that being exposed to concept relations (Q2) increase complexity such that the user interface becomes less manageable (Q7). However, participants still found that relation information was useful for the exploratory task. Therefore, users expressed a preferences for GRAFS because, if given more time on task, it would support a  deeper understanding of the topic during exploratory literature search. In this way, participants' preference for GRAFS can be viewed as evidence for \textbf{Hypothesis 1}.

\subsubsection{Participants' Feedback on Factors Affecting the Generated Outlines}

During the exit interviews, participants provided detailed reasons for why they preferred the outline they generated with one system over the other when answering I1.  Participants' comments indicate that the interface design did effect their activity when completing the task, but the influence of search topic on a user's outline proved to be larger. This may help explain why we did not observe major differences in the quality of people's outlines in A1, A2, A5, and A6 (Section \ref{sec:Outline Task objective}).
% Therefore, \textbf{Hypothesis 1.b} might be very difficult to test.
 
Reflecting this, most of the participants ($n = 12$) mentioned the influence of topic difference on the outline quality. This include the technicality of a topic, participants' familiarity with a topic, and whether a topic is evolving or well-established. Some participants ($n = 6$) thought ``Treatment for Depression'' was easier than ``COVID-19 Diagnosis'' in terms of vocabulary and the topic's structure. Five participants mentioned that they were more familiar with one of the topics, and those participants felt that they did a better job on the familiar topic. Some participants ($n=4$) mentioned that the two topics were different from each other in the work required to perform the task, which in turn influenced the quality of the final outcomes. Three out of the four participants commented that they found depression to be a well-established field while COVID-19 related research was newer (and therefore harder to approach due to the more scattered and heterogeneous set of related concepts).
% For instance, User 12 mentioned that he had a better idea of how to approach the topic of depression, while the covid topic has a lot of new concepts and he didn't know how to start.

% As described by User 16, "For depression, there are much more evidence, studies, and clinical trials." Therefore, she was able to read more articles with more "systematic and analytical results" and saw the comparison between different treatment methods. But for COVID-19, "most of the articles only present simple findings". Therefore, her outline of covid was more like a simple list of methods she found. 

A number of participants ($n=6$) mentioned that the features of the interface affected the quality of their outline. Four users said that GRAFS helped them generate good summaries as it enabled them to edit the concept list ($n=2$), see relations between concepts ($n=1$), and was easier to use ($n=1$). In contrast, one participant thought the features in GRAFS were distracting and negatively influenced his work. One participant liked the categories given in the baseline system and reported that they helped her to write a good summary.
% This illustrates that participants prefer GRAFS for exploratory search, but GRAFS may not necessarily help with the outcome of the task. We seek to further understand this phenomenon through interview analysis in section 5.4.1 and 5.4.2.

Overall, we found that topic difference and participants’ background may have a bigger impact on outline quality than the system. On the one hand, these factors may exaggerate the number of votes given to one system versus another due to the small sample size of the study. On the other hand, these factors may also obscure system differences (e.g. if participants always perform better on one topic, then GRAFS and Baseline will always get equal votes).

\subsection{Question-Answering Task}
\label{sec:Question-Answering Task}
Participants indicated their perception of the difficulty of the question answering task through the post-task questionnaire. As mentioned in Section \ref{sec:result overview}, there is no significant difference between the ratings given to the two systems regarding the task's difficulty ($p=0.510$). We further evaluated participants' performance based on the time spent on the task. On average, participants spent 181.1s on question answering task using GRAFS and 238.2s using the baseline system, and the difference is not significant ($p=0.208$). This shows that participants performed the question answering task at least as well on GRAFS as on a typical faceted search system, which supports \textbf{Hypothesis 2.a}.


\subsection{Qualitative User Feedback}
\label{sec:Qualitative User Feedback}

\subsubsection{Benefits of GRAFS and Baseline}
\label{sec:Benefits of GRAFS and baseline}
% May give some examples for each of the feedback mentioned 

As mentioned in Section \ref{sec:Outline Task subjective}, the majority of participants preferred GRAFS over the baseline system (14:6). During the exit interview, we asked participants to indicate the reason of their preference. In general, participants' feedback shows that the new information and functions provided by GRAFS facilitated users' exploratory activity, while introducing some complexity to the system. 

Participants described benefits of GRAFS related to: (1) relations, (2) specific components, and (3) general experience. Several users ($n=4$) mentioned that they loved the fact that they can learn relations between concepts in GRAFS (\textbf{Hypothesis 1.a}). Many participants ($n=7$) mentioned some components that they particularly liked, including facet treemap ($n=4$), editable list ($n=3$), and facet list arcs ($n=3$). Four participants selected GRAFS for a better overall experience. Specifically, they mentioned GRAFS is interesting and colorful ($n=2$), and helps with overview ($n=1$) and new ideas ($n=1$). These comments reflect that a majority of the participants found the newly introduced components usable and were able to apply those new information into their tasks, providing support for \textbf{Hypothesis 2.b}.

Most of the participants that preferred the baseline system thought the baseline system is clearer ($n=4$), while two mentioned that they liked the pre-defined categories ($n=2$).
% For instance, User 2 said that she preferred GRAFS mainly because she can edit the concept list in this system.

% \subsubsection{Factors Affecting the Generated Outlines}
% \label{sec:Evaluation of Generated Outlines}
% % While most of the participants appreciated the new information and function provided in GRAFS, we didn't observe major difference in the quality of people's outlines except for documentation and depth. When asked which outline they preferred, most of the participants selected the outline generated using the baseline system (baseline: 12, GRAFS: 7, no difference: 1). 
% During the exit interview, we asked users which outline were they more satisfied with between the two they generated using GRAFS and the Baseline and why they preferred one over the other.  Participants' comments indicate that the interface design did effect their activity when completing the task, but the influence of search topic on a user's outline proved to be larger. This may help explain why we did not observe major differences in the quality of people's outlines except in the aspects of documentation (A4) and depth (A3) (Section \ref{sec:Outline Task}).
 
% Reflecting this, most of the participants ($n=12$) mentioned the influence of topic difference on the outline quality, including difficulty, familiarity, emerging vs established, and certainty of the results. Some participants ($n=6$) thought ``Treatment for Depression'' was easier than ``COVID-19 Diagnosis'' in terms of vocabulary and the topic's structure. Five participants mentioned that they were more familiar with one of the topics, and those participants felt that they did a better job on the familiar topic. Some participants ($n=4$) mentioned that the two topics were different from each other in the work required to perform the task, which in turn influenced the quality of the final outcomes. Three out of the four participants commented that they found depression to be a well-established field while COVID-19 related research was newer (and therefore harder to approach due to the more scattered and heterogeneous set of related concepts).

% A number of participants ($n=6$) mentioned that the features of the interface affected the quality of their outline. Four users said that GRAFS helped them generate good summaries as it enabled them to edit the concept list ($n=2$), see relations between concepts ($n=1$), and was easier to use ($n=1$). In contrast, one participant thought the features in GRAFS were distracting and negatively influenced his work. One participant liked the categories given in the baseline system and helped her to write good summary. 



\subsubsection{Usability of Interface Features}
\label{sec:Usability of interface features}
%This section reports on the feedback collected focusing on each components we introduced in GRAFS to further test \textbf{Hypothesis 2.b}. 

During the exit interview, participants were asked whether a component is useful or not for accomplishing the given tasks.  We note that there is a difference between (1) a participant not using a feature, and (2) a participant finding the feature not useful after using it. More specifically, we noticed that some participants did not use certain features in GRAFS due to time limitation, lack of domain knowledge, and limited experience with a new interface design.
Therefore, we report both (1) the number of participants that used each feature based on the action log, and (2) the number of participants that found each feature to be useful. 

Overall, the facet list arcs were the most used feature. The facet treemap was used less often, in part due to its higher complexity. The functions of deleting and adding concepts were least used. Though they all add complexity to the traditional faceted search interface, the components all received positive feedback from participants who have used them. The concept provenance tooltip was found to be easy to use, but not as useful as other components.
% We focus on \textit{concept arcs}, \textit{concept treemap}, \textit{concept grounding examples}, \textit{editable list}.
% An overview of the use of components is show in table \ref{tab:components}.

% \begin{table}[H]
%     \centering
%     \begin{tabular}{c|c|c|c}
%          \hline
%                                                                     & Useful & Not Useful & No Indication \\ \hline
% Concept Arcs                                                        & 11     & 9          & 0             \\ \hline
% Concept Treemap                                                     & 9      & 11         & 0             \\ \hline
% \begin{tabular}[c]{@{}c@{}}Concept Grounding\\ Tooltip\end{tabular} & 8      & 11         & 1             \\ \hline
% \begin{tabular}[c]{@{}c@{}}Editable List\\ Delete\end{tabular}      & 6      & 13         & 1             \\ \hline
% \begin{tabular}[c]{@{}c@{}}Editable List\\ Add\end{tabular}         & 4      & 15         & 1             \\ \hline
%     \end{tabular}
%     \caption{Use of components}
%     \label{tab:components}
% \end{table}

\textbf{Facet List Arcs:} Action logs show that all 20 participants made at least one selection from the facet list, which triggers the display of facet list arcs. The majority of participants thought the feature of concept arcs to be useful ($n=11$). Some participants ($n=6$) mentioned that arcs helped inform them about what to look at or which concepts to click next (\textbf{Hypothesis 1.b}). Five participants mentioned that arcs helped them understand relations between concepts (\textbf{Hypothesis 1.a}), which in turn helped them better understand the topic and adjust their selection strategy (\textbf{Hypothesis 1.b}). 
%Overall, these findings suggest that arcs encouraged participants' exploration and facilitated their understanding of the relations between concepts.

% For instance, User 7 said that he is not familiar with the topic, so the arcs helped him "see the basic idea of the topic and see what to pay attention to" and it’s "especially helpful during the initial exploration". One possible drawback mentioned by one of the participants is that arcs were repeatedly drawn between some concepts. Though the participant already examined that relation, her attention were still attracted to it, which is distracting. 

For participants that did not state that arcs were useful, a majority of them said that they ignored this feature ($n=5$). For instance, User 4 said that he preferred to just read articles and User 12 mentioned that due to time limitations, he was not able to use that information. Some participants ($n=2$) used alternatives to the arcs to get similar information, such as the facet treemap, or the number of documents listed near each concept.

\textbf{Facet Treemap:} We considered a participant to have used the facet treemap if they clicked at least once on a concept in the visualization. 13 participants meet this criterion. Participant feedback illustrates that the facet treemap can be difficult to make sense of due to its unfamiliarity, and it introduces complexity to using the system. Yet while it may take time for users to learn how to use this feature, nine out of 20 participants thought that the facet treemap was useful. 

Most of the participants who found it useful ($n=8$) reported that the facet treemap helped them see the relations between concepts (\textbf{Hypothesis 1.a}). Because both the facet treemap and the facet list arcs communicate the connections between concepts, some participants ($n=7$) compared the two. Five participants indicated that they preferred facet treemap compared to facet list arcs, while the other two participants preferred arcs. Those two felt that the arcs were more straightforward. 

Interestingly, among people that preferred the facet treemap, two participants commented that facet treemap was not straightforward to understand and that it took time for them to find it useful. For instance, User 20 mentioned that he didn’t find treemap to be useful immediately. However, during the exploration, he found that thick arcs in the facet list always seemed to connect to broader concepts such as infectious disease. He therefore started to look to the treemap for a more nuanced view of the relations and, eventually, found the treemap to be more useful. User 14 mentioned that at the beginning of the session, she felt the information in the facet treemap is cluttered and the structure seemed to be quite complex. As a result, she assumed that it would be hard to understand the treemap and ignored it. Only after using the facet treemap did she realized that it is easy to use.

% Some participants (n=2) also found that treemap is easy to click and good for navigation. One participants thought treemap can provide an overview of the topic.

A majority of the participants ($n=11$) did not report the facet treemap as being useful. Three participants felt the information was cluttered and overwhelming, while some participants ($n=2$) thought it occupied too much screen space. Three participants mentioned that it was difficult to make sense of the information provided by the facet treemap, and two participants said they were not used to information presented in that way. Many of these comments suggest unfamiliarity as a key hurdle.

\textbf{Concept Provenance Tooltip:} All participants used this feature when hovering over items in the facet list. Eight participants mentioned that the facet list tooltip was useful. Some participants ($n=4$) mentioned that the tooltip helped them gain a quick understanding of what the concept meant. Two participants expressed the wish that they could navigate directly to an original article from the given examples. 

For people that did not report that the facet list tooltip was useful, four mentioned that they did not need extra explanations of the concepts either because they had good background knowledge or they only used familiar concepts during their exploration. Some participants ($n=3$) preferred to understand concepts using other method, such as ``googling'' or reading the actual articles. One participant mentioned that the usefulness of the tooltip was highly dependent on the content of the sentence shown in the tooltip. Overall, the concept provenance tooltips were found to help people understand concepts during exploration, but only when users were faced with new concepts.
% During the exit interview, we focused on the concept grounding tooltip shown next to the concept list. 

\textbf{Editable List:} GRAFS allows users to make adjustments to the automatically generated knowledge subgraph by deleting or adding concepts. Overall, this feature was less used by participants due to task time  constraint, limited familiarity with the topic, and limited training with this way of interacting. However, participants provided positive feedback on this feature, and we found some interesting use cases that indicate the benefits of preserving human agency in GRAFS.

In total, seven participants used the function of either deleting or adding concepts. Out of these seven, four participants used both, two participants only deleted concepts, and one participant only added concepts.

We examine the feedback regarding deleting concepts and adding concepts separately. Six of the 20 participants used the function of deleting concepts, and six participants (four of the six participants that used concept deletion, plus two who did not use concept deletion) mentioned that the function of deleting concepts was useful for removing irrelevant or equivalent variants of concepts. This helped users focus on a shortened concept list ($n=2$) and find important relations faster ($n=1$). 

Five of the 20 participants used the function of adding concepts, and four participants (three of the five participants that used concept addition, plus one who did not use concept addition) found adding concepts to be useful. Two people used this function when they came across unlisted concepts that they felt were important based on their reading. An interesting use case was provided by User 2. She described that when she worked on ``Treatment for Depression,'' she frequently came across the concept of ``Exercise.'' Therefore, she added ``Exercise'' to the concept list to investigate deeper. When she felt she had done enough reading of related materials, she then removed the concept from the list. One participant added the concept ``COVID-19,'' which was removed as a per-query stop word, to remind herself about the major topic. One participant suggested the interface should enable users to add new concepts to the facet list by directly typing in concept names in addition to selecting concepts in documents.

For participants that did not use the add or remove functions, four participants mentioned that time limitation was a major reason. Some participants ($n=3$) mentioned that the lack of familiarity with the topic is another important factor. 

% For instance, User 10 said that he "likes the fact that he can add new concepts into the concept list", though he didn’t use that function during the study, he "can imagine using that function if I spend a whole day to write the summary." 
% For instance, User 9 mentioned that she was not familiar with the concepts. But if she knew what she wanted, she "will be able to delete some concepts to shorten the list and be more focused." Besides, another two participants suggested that they wanted to customize concepts to add into the list.

% \subsection{Additional Analysis}
% % further analysis
% \subsubsection{Influential Factors}
% People's perceptions of the both GRAFS and the baseline faceted search system may vary with their background and the order of using the systems. In our analysis, we split participants into groups considering the order of using the two systems ($G_{order}$), whether they have biomedical domain knowledge ($G_{domain}$), experience of conducting a literature review ($G_{experience}$), and topic familiarity ($G_{familiar}$). We evaluated the effects of these group identities on the questionnaire responses that had statistically significant findings (Q2 relation, Q7 manageable, and Q8 stimulating) with a mixed ANOVA model. The group identities were treated as between-subject factors and the system (GRAFS or baseline) was treated as a within-subject factor. 
% \begin{table}[h]
% \begin{tabular}{llll}
% \hline
%                     & F     & $\eta^2$ & p     \\ \hline
% $G_{order}$        & 0.323 & 0.018  & 0.577 \\ 
% $System$              & 6.406 & 0.262  & 0.021 \\ 
% $G_{order}\times System$ & 3.139 & 0.148  & 0.093 \\ \hline
% \end{tabular}
% \caption{Effect of order on a user's rating of relation}
% \label{tab:order_effect}
% \end{table}

% \begin{table}[h]
% \begin{tabular}{llll}
% \hline
%                     & F     & $\eta^2$ & p     \\ \hline
% $G_{domain}$       & 6.170 & 0.255  & 0.023 \\ 
% $System$              & 1.797 & 0.091  & 0.197 \\ 
% $G_{domain}\times System$ & 0.002 & 0.000  & 0.967 \\ \hline
% \end{tabular}
% \caption{Effect of domain knowledge on a user's rating of easy to use}
% \label{tab:knowledge_effect1}
% \end{table}

% \begin{table}[h]
% \begin{tabular}{llll}
% \hline
%                     & F     & $\eta^2$ & p     \\ \hline
% $G_{domain}$       & 8.160 & 0.312  & 0.010 \\ 
% $System$              & 3.635 & 0.168  & 0.073 \\ 
% $G_{domain}\times System$ & 0.173 & 0.010  & 0.682 \\ \hline
% \end{tabular}
% \caption{Effect of domain knowledge on a user's rating of manageable}
% \label{tab:knowledge_effect2}
% \end{table}

% \begin{figure}[t]
% \centering  
% \includegraphics[width=1\textwidth]{fig/result_effect.pdf}
% \Description[result1]{result1}
% \caption{The effects of the order of using the two systems and participants' domain knowledge on participants' perception of the system. (a) Participants that worked on GRAFS first gave lower scores to the baseline in the system's ability to help them see the relation between concepts. (b) Biomedical domain experts gave higher scores to ``easy to use'' compared to participants without domain knowledge. (c) Biomedical domain experts gave higher scores to ``Manageable'' compared to participants without domain knowledge.}
% \label{fig:res_effect}
% \end{figure}

% Topic familiarity and literature search experience did not have any effect on participants' ratings. A significant interaction effect between the order and system was found for participants' rating on the relation (p<0.1, Table \ref{tab:order_effect}). As shown in Figure \ref{fig:res_effect}(a), when rating whether the system helps to see concept relations, people that worked on GRAFS first tend to give lower scores to the baseline system compared to the case when the user started from the baseline system. This phenomenon indicates that users did use some of the provided visual representations in GRAFS to perceive the relations between concepts. When exposed to the baseline system as the second interface, users appeared to have an increased awareness of the difficulty in seeing concept relations without the GRAFS features. This further supports our \textbf{Hypothesis 1}. 
% % (a table, post hoc?)
% Additionally, participants with biomedical background gave significantly higher scores for the question of easy to use (Table \ref{tab:knowledge_effect1}, Figure \ref{fig:res_effect}(b)) and manageable (Table \ref{tab:knowledge_effect2}, Figure \ref{fig:res_effect}(c)) for both GRAFS and the baseline system. The effect of $G_{domain}$ is more significant than the effect of the system on the two questions. This shows that people's judgement of a system's usability is highly influenced by people's domain knowledge.

% \subsubsection{Compare concept selection behaviors of the two systems}




